Covers of surfaces

We study the homeomorphism types of certain covers of (always orientable) surfaces, usually of infinite-type. We show that every surface with non-abelian fundamental group is covered by every noncompact surface, we identify the universal abelian covers and the $\mathbb{Z}/n\mathbb{Z}$-homology covers of surfaces, and we show that non-locally finite characteristic covers of surfaces have four possible homeomorphism types.

==> figures/covers-figures <==
<?xml version="1.0" encoding="UTF-8" standalone="no"?>
<!-- Created with Inkscape (http://www.inkscape.org/) -->

<svg
   width="626.70953mm"
   height="135.91495mm"
   viewBox="0 0 626.70953 135.91495"
   version="1.1"
   id="svg1"
   xml:space="preserve"
   inkscape:version="1.3.2 (091e20e, 2023-11-25, custom)"
   sodipodi:docname="short curves figures.svg"
   inkscape:export-filename="flute.png"
   inkscape:export-xdpi="96"
   inkscape:export-ydpi="96"
   xmlns:inkscape="http://www.inkscape.org/namespaces/inkscape"
   xmlns:sodipodi="http://sodipodi.sourceforge.net/DTD/sodipodi-0.dtd"
   xmlns:xlink="http://www.w3.org/1999/xlink"
   xmlns="http://www.w3.org/2000/svg"
   xmlns:svg="http://www.w3.org/2000/svg"><sodipodi:namedview
     id="namedview1"
     pagecolor="#ffffff"
     bordercolor="#000000"
     borderopacity="0.25"
     inkscape:showpageshadow="2"
     inkscape:pageopacity="0.0"
     inkscape:pagecheckerboard="0"
     inkscape:deskcolor="#d1d1d1"
     inkscape:document-units="px"
     showguides="false"
     inkscape:zoom="0.64558333"
     inkscape:cx="3115.7868"
     inkscape:cy="642.82948"
     inkscape:window-width="1730"
     inkscape:window-height="1032"
     inkscape:window-x="172"
     inkscape:window-y="0"
     inkscape:window-maximized="0"
     inkscape:current-layer="g208"
     showgrid="false"
     inkscape:export-bgcolor="#ffffffff"><sodipodi:guide
       position="-198.47838,1411.6708"
       orientation="1,0"
       id="guide4"
       inkscape:locked="false" /><sodipodi:guide
       position="360.88761,1210.154"
       orientation="0,-1"
       id="guide5"
       inkscape:locked="false" /><sodipodi:guide
       position="-63.338372,1303.4241"
       orientation="1,0"
       id="guide1"
       inkscape:locked="false" /><sodipodi:guide
       position="-556.26955,1519.44"
       orientation="1,0"
       id="guide2"
       inkscape:locked="false" /><sodipodi:guide
       position="117.2034,1146.9195"
       orientation="0,-1"
       id="guide41"
       inkscape:locked="false" /><sodipodi:guide
       position="291.553,1041.6027"
       orientation="0,-1"
       id="guide57"
       inkscape:locked="false" /><sodipodi:guide
       position="358.44151,1461.1102"
       orientation="0,-1"
       id="guide91"
       inkscape:locked="false" /><sodipodi:guide
       position="181.04147,1525.0906"
       orientation="0,-1"
       id="guide92"
       inkscape:locked="false" /><sodipodi:guide
       position="180.41661,1449.0891"
       orientation="0,-1"
       id="guide218"
       inkscape:locked="false" /><sodipodi:guide
       position="335.18248,1536.6086"
       orientation="1,0"
       id="guide322"
       inkscape:locked="false" /><inkscape:grid
       id="grid338"
       units="px"
       originx="-656.51959"
       originy="-127.60464"
       spacingx="0.26458333"
       spacingy="0.26458333"
       empcolor="#0099e5"
       empopacity="0.30196078"
       color="#0099e5"
       opacity="0.14901961"
       empspacing="5"
       dotted="false"
       gridanglex="30"
       gridanglez="30"
       visible="false" /><sodipodi:guide
       position="136.92301,1544.4078"
       orientation="1,0"
       id="guide338"
       inkscape:locked="false" /><sodipodi:guide
       position="269.89157,1534.0381"
       orientation="1,0"
       id="guide339"
       inkscape:locked="false" /><sodipodi:guide
       position="253.44034,1471.8318"
       orientation="0,-1"
       id="guide342"
       inkscape:locked="false" /><sodipodi:guide
       position="467.82071,1545.3483"
       orientation="1,0"
       id="guide347"
       inkscape:locked="false" /><sodipodi:guide
       position="309.47742,1234.3168"
       orientation="0,-1"
       id="guide109"
       inkscape:locked="false" /><sodipodi:guide
       position="402.01571,1552.5457"
       orientation="1,0"
       id="guide126"
       inkscape:locked="false" /><sodipodi:guide
       position="19.636468,1498.9168"
       orientation="1,0"
       id="guide193"
       inkscape:locked="false" /><sodipodi:guide
       position="102.61099,1396.3119"
       orientation="0,-1"
       id="guide208"
       inkscape:locked="false" /><sodipodi:guide
       position="533.62571,1556.6585"
       orientation="1,0"
       id="guide209"
       inkscape:locked="false" /><sodipodi:guide
       position="599.94481,1553.5739"
       orientation="1,0"
       id="guide210"
       inkscape:locked="false" /><sodipodi:guide
       position="665.74981,1542.2637"
       orientation="1,0"
       id="guide211"
       inkscape:locked="false" /><sodipodi:guide
       position="203.31645,1557.5226"
       orientation="1,0"
       id="guide233"
       inkscape:locked="false" /><sodipodi:guide
       position="70.939408,1547.6865"
       orientation="1,0"
       id="guide234"
       inkscape:locked="false" /></sodipodi:namedview><defs
     id="defs1"><inkscape:path-effect
       effect="spiro"
       id="path-effect339"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect290"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect288"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect277"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect275"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect273"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect271"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect269"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect267"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect260"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect258"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect256"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect254"
       is_visible="true"
       lpeversion="1" /><linearGradient
       id="linearGradient232"
       inkscape:collect="always"><stop
         style="stop-color:#fdfdfd;stop-opacity:1;"
         offset="0"
         id="stop232" /><stop
         style="stop-color:#a58eab;stop-opacity:0;"
         offset="1"
         id="stop233" /></linearGradient><inkscape:path-effect
       effect="spiro"
       id="path-effect208"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect190"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect186"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect184"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect182"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect180"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect178"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect175"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect172"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect170"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect168"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect154"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect152"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect149"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect146"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect144"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect142"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect140"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect138"
       is_visible="true"
       lpeversion="1" /><rect
       x="3668.4517"
       y="1019.4723"
       width="79.689209"
       height="107.16825"
       id="rect198" /><rect
       x="3660.208"
       y="1035.9597"
       width="90.680824"
       height="96.176636"
       id="rect197" /><inkscape:path-effect
       effect="spiro"
       id="path-effect189"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect187"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect176"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect174"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect163"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect161"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect150"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect148"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect123"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect121"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect116"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect114"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect109"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect299"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect297"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect251"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect249"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect247"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect245"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect229"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect227"
       is_visible="true"
       lpeversion="1" /><linearGradient
       id="linearGradient209-1"><stop
         style="stop-color:#8150bc;stop-opacity:0;"
         offset="0.42369023"
         id="stop206" /><stop
         style="stop-color:#80449e;stop-opacity:0.26480839;"
         offset="0.84619027"
         id="stop209" /></linearGradient><linearGradient
       id="linearGradient205"><stop
         style="stop-color:#2a2a2a;stop-opacity:1;"
         offset="0.04328017"
         id="stop202" /><stop
         style="stop-color:#151515;stop-opacity:0.49803922;"
         offset="0.12072892"
         id="stop203" /><stop
         style="stop-color:#0a0a0a;stop-opacity:0.24705882;"
         offset="0.21981776"
         id="stop204" /><stop
         style="stop-color:#000000;stop-opacity:0;"
         offset="0.56036437"
         id="stop205" /></linearGradient><linearGradient
       id="linearGradient189-1"><stop
         style="stop-color:#2a2a2a;stop-opacity:1;"
         offset="0.04328017"
         id="stop189" /><stop
         style="stop-color:#151515;stop-opacity:0.49803922;"
         offset="0.14806378"
         id="stop193" /><stop
         style="stop-color:#0a0a0a;stop-opacity:0.24705882;"
         offset="0.39977217"
         id="stop194" /><stop
         style="stop-color:#000000;stop-opacity:0;"
         offset="0.87015939"
         id="stop190" /></linearGradient><linearGradient
       id="swatch95"
       inkscape:swatch="solid"><stop
         style="stop-color:#000000;stop-opacity:1;"
         offset="0"
         id="stop95" /></linearGradient><inkscape:path-effect
       effect="spiro"
       id="path-effect70"
       is_visible="true"
       lpeversion="1" /><inkscape:path-effect
       effect="spiro"
       id="path-effect68"
       is_visible="true"
       lpeversion="1" /><marker
       style="overflow:visible"
       id="ArrowWideRounded"
       refX="0"
       refY="0"
       orient="auto-start-reverse"
       inkscape:stockid="Wide, rounded arrow"
       markerWidth="1"
       markerHeight="1"
       viewBox="0 0 1 1"
       inkscape:isstock="true"
       inkscape:collect="always"
       preserveAspectRatio="xMidYMid"><path
         style="fill:none;stroke:context-stroke;stroke-width:1;stroke-linecap:round"
         d="M 3,-3 0,0 3,3"
         transform="rotate(180,0.125,0)"
         sodipodi:nodetypes="ccc"
         id="path2" /></marker><marker
       style="overflow:visible"
       id="Triangle"
       refX="0"
       refY="0"
       orient="auto-start-reverse"
       inkscape:stockid="Triangle arrow"
       markerWidth="8"
       markerHeight="8"
       viewBox="0 0 1 1"
       inkscape:isstock="true"
       inkscape:collect="always"
       preserveAspectRatio="xMidYMid"><path
         transform="scale(0.5)"
         style="fill:context-stroke;fill-rule:evenodd;stroke:context-stroke;stroke-width:1pt"
         d="M 5.77,0 -2.88,5 V -5 Z"
         id="path135" /></marker><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient201"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient202"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient209"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       gradientUnits="userSpaceOnUse"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient211"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><clipPath
       clipPathUnits="userSpaceOnUse"
       id="clipPath217"><ellipse
         style="display:inline;fill:#1a1a1a;fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
         id="ellipse217"
         cx="787.11633"
         cy="292.62439"
         rx="45.074406"
         ry="42.48214" /></clipPath><clipPath
       clipPathUnits="userSpaceOnUse"
       id="clipPath218"><ellipse
         style="display:inline;fill:#1a1a1a;fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
         id="ellipse218"
         cx="787.11633"
         cy="292.62439"
         rx="45.074406"
         ry="42.48214" /></clipPath><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient229"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient230"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient230"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient231"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient261"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient262"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient262"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient263"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient263"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient264"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient264"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient265"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient308"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient309"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient123"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient124"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient125"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient126"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient150"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient151"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient151"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient152"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient163"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient164"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient164"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient165"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient176"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient177"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient177"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient178"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient191"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient192"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient192"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient193"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><inkscape:path-effect
       effect="spiro"
       id="path-effect208-4"
       is_visible="true"
       lpeversion="1" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient232"
       id="linearGradient233"
       x1="915.08051"
       y1="452.17328"
       x2="915.58771"
       y2="317.43729"
       gradientUnits="userSpaceOnUse" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient340"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient341"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient341"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient342"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient342"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient343"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient343"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient344"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient344"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient345"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient345"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient346"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient347"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient348"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient348"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient349"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient349"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient350"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient350"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient351"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient351"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient352"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient352"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient353"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient353"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient354"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient354"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient355"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient355"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient356"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient189-1"
       id="linearGradient356"
       gradientUnits="userSpaceOnUse"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><linearGradient
       inkscape:collect="always"
       xlink:href="#linearGradient205"
       id="linearGradient357"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1,0,0,1,1570.9832,-0.38573878)"
       x1="814.2547"
       y1="297.07309"
       x2="811.95068"
       y2="277.01468"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient357"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(1.7938226,-0.36445534,0.22075605,1.0963785,-698.65472,266.93209)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /><radialGradient
       inkscape:collect="always"
       xlink:href="#linearGradient209-1"
       id="radialGradient358"
       gradientUnits="userSpaceOnUse"
       gradientTransform="matrix(-1.7938226,-0.36445534,-0.22075605,1.0963785,2268.8801,267.15805)"
       cx="808.08575"
       cy="271.95767"
       fx="808.08575"
       fy="271.95767"
       r="23.38006"
       spreadMethod="reflect" /></defs><g
     id="g338"
     inkscape:label="FIGURE inf type cover"
     style="display:none"
     transform="translate(-656.51959,-127.60463)"><g
       id="g80"
       inkscape:label="generaINF TYPE"
       style="display:inline;stroke-width:1.4006;stroke-dasharray:none"
       transform="matrix(0.94666662,0,0,0.94241181,163.4309,-78.572482)"
       inkscape:export-filename="..\Documents\TEX FILES\research what am i doing\short curves\fig\rholadder.png"
       inkscape:export-xdpi="96"
       inkscape:export-ydpi="96"><path
         style="fill:#1a1a1a;stroke:#000000;stroke-width:1.4006;stroke-dasharray:none"
         d="M 572.33152,357.24836 1293.493,356.47688"
         id="path92"
         sodipodi:nodetypes="cc"
         inkscape:label="surface line bottom" /><path
         style="display:inline;fill:#1a1a1a;stroke:#000000;stroke-width:1.4006;stroke-dasharray:none"
         d="M 571.56351,228.41161 1292.725,227.64013"
         id="path91"
         sodipodi:nodetypes="cc"
         inkscape:label="surface line" /><g
         id="g231"
         style="display:none;stroke-width:1.61117;stroke-dasharray:none"
         inkscape:label="double genus"
         transform="matrix(0.92836947,0,0,0.81400337,67.318693,52.198656)"><g
           id="g226"
           inkscape:label="shadow genus together now1"
           style="display:inline;stroke-width:1.61117;stroke-dasharray:none"
           transform="translate(18.432243,1.1572163)"><path
             style="display:none;fill:url(#linearGradient229);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
             id="path220"
             inkscape:label="shadowR"
             sodipodi:nodetypes="cccccc" /><path
             style="display:none;fill:url(#linearGradient230);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
             id="path221"
             inkscape:label="shadowL"
             sodipodi:nodetypes="cccccc" /><path
             style="display:inline;fill:url(#radialGradient230);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
             id="path222"
             inkscape:label="shadowR"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)"
             clip-path="url(#clipPath218)" /><path
             style="display:inline;fill:url(#radialGradient231);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
             id="path223"
             inkscape:label="shadowL purp"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)"
             clip-path="url(#clipPath217)" /><g
             id="g225"
             inkscape:label="genus hole 1"
             style="display:inline;stroke-width:1.63241;stroke-dasharray:none"
             transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
               style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
               id="path224"
               inkscape:path-effect="#path-effect227"
               inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
               transform="translate(311.23778,-33.331065)"
               sodipodi:nodetypes="cscc" /><path
               style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
               id="path225"
               inkscape:path-effect="#path-effect229"
               inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
               sodipodi:nodetypes="cssc"
               transform="translate(310.49613,-35.888171)" /></g></g></g><g
         id="g244"
         style="display:none;stroke-width:1.61117;stroke-dasharray:none"
         inkscape:label="double genus"
         transform="matrix(0.92836947,0,0,0.81400337,277.76424,51.209087)"><g
           id="g237"
           inkscape:label="shadow genus together now"
           style="display:inline;stroke-width:1.61117;stroke-dasharray:none"
           transform="translate(165.3405,1.8294203)"><path
             style="display:none;fill:url(#linearGradient261);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
             id="path231"
             inkscape:label="shadowR"
             sodipodi:nodetypes="cccccc" /><path
             style="display:none;fill:url(#linearGradient262);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
             id="path232"
             inkscape:label="shadowL"
             sodipodi:nodetypes="cccccc" /><path
             style="display:inline;fill:url(#radialGradient262);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
             id="path233"
             inkscape:label="shadowR"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)"
             clip-path="url(#clipPath218)" /><path
             style="display:inline;fill:url(#radialGradient263);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
             id="path234"
             inkscape:label="shadowL purp"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)"
             clip-path="url(#clipPath217)" /><g
             id="g236"
             inkscape:label="genus hole 1"
             style="display:inline;stroke-width:1.63241;stroke-dasharray:none"
             transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
               style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
               id="path235"
               inkscape:path-effect="#path-effect245"
               inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
               transform="translate(311.23778,-33.331065)"
               sodipodi:nodetypes="cscc" /><path
               style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
               id="path236"
               inkscape:path-effect="#path-effect247"
               inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
               sodipodi:nodetypes="cssc"
               transform="translate(310.49613,-35.888171)" /></g></g><g
           id="g243"
           inkscape:label="shadow genus together now1"
           style="display:inline;stroke-width:1.61117;stroke-dasharray:none"
           transform="translate(39.936526,1.9286938)"><path
             style="display:none;fill:url(#linearGradient263);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
             id="path237"
             inkscape:label="shadowR"
             sodipodi:nodetypes="cccccc" /><path
             style="display:none;fill:url(#linearGradient264);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
             id="path238"
             inkscape:label="shadowL"
             sodipodi:nodetypes="cccccc" /><path
             style="display:inline;fill:url(#radialGradient264);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
             id="path239"
             inkscape:label="shadowR"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)"
             clip-path="url(#clipPath218)" /><path
             style="display:inline;fill:url(#radialGradient265);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
             id="path240"
             inkscape:label="shadowL purp"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)"
             clip-path="url(#clipPath217)" /><g
             id="g242"
             inkscape:label="genus hole 1"
             style="display:inline;stroke-width:1.63241;stroke-dasharray:none"
             transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
               style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
               id="path241"
               inkscape:path-effect="#path-effect249"
               inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
               transform="translate(311.23778,-33.331065)"
               sodipodi:nodetypes="cscc" /><path
               style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
               id="path242"
               inkscape:path-effect="#path-effect251"
               inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
               sodipodi:nodetypes="cssc"
               transform="translate(310.49613,-35.888171)" /></g></g></g><g
         id="g113"
         inkscape:label="single genus "
         style="display:none;stroke-width:1.61117;stroke-dasharray:none"
         transform="matrix(0.92836947,0,0,0.81400337,-35.60405,51.707014)"><path
           style="display:inline;fill:url(#radialGradient308);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path109"
           inkscape:label="shadowR"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath218)" /><path
           style="display:inline;fill:url(#radialGradient309);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path110"
           inkscape:label="shadowL purp"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath217)" /><g
           id="g112"
           inkscape:label="genus hole 1"
           style="display:inline;stroke-width:1.63241;stroke-dasharray:none"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path111"
             inkscape:path-effect="#path-effect114"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             transform="translate(311.23778,-33.331065)"
             sodipodi:nodetypes="cscc" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path112"
             inkscape:path-effect="#path-effect116"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g></g><g
       id="g49"
       inkscape:label="Fin TYPEGenus"
       style="display:inline;stroke-width:1.4006;stroke-dasharray:none"
       transform="matrix(0.94666662,0,0,0.94241181,638.18752,-98.878207)"><g
         inkscape:groupmode="layer"
         id="g48"
         inkscape:label="arrow"
         style="display:none;stroke-width:1.4006;stroke-dasharray:none"><path
           style="display:inline;opacity:1;fill:none;stroke:#000000;stroke-width:1.4006;stroke-dasharray:none;stroke-dashoffset:0;stroke-opacity:1"
           d="m 453.36702,398.79707 c 0,55.58188 0.65839,55.58188 0.65839,55.58188"
           id="path47"
           inkscape:label="tail" /><path
           style="opacity:1;fill:none;stroke:#000000;stroke-width:1.4006;stroke-dasharray:none;stroke-dashoffset:0;stroke-opacity:1"
           d="m 448.04429,447.499 5.63464,6.90696 5.63463,-7.08873"
           id="path48"
           sodipodi:nodetypes="ccc"
           inkscape:label="head" /></g><g
         id="g296"
         inkscape:label="single genus "
         style="display:inline;stroke-width:1.805;stroke-dasharray:none"
         transform="matrix(0.7710386,0,0,0.7809002,-254.89378,370.19338)"><path
           style="display:inline;fill:url(#radialGradient123);fill-opacity:1;stroke:none;stroke-width:1.8288;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path292"
           inkscape:label="shadowR"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath218)" /><path
           style="display:inline;fill:url(#radialGradient124);fill-opacity:1;stroke:none;stroke-width:1.8288;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path293"
           inkscape:label="shadowL purp"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath217)" /><g
           id="g295"
           inkscape:label="genus hole 1"
           style="display:inline;stroke-width:1.8288;stroke-dasharray:none"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.8288;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path294"
             inkscape:path-effect="#path-effect297"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             transform="translate(311.23778,-33.331065)"
             sodipodi:nodetypes="cscc" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.8288;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path295"
             inkscape:path-effect="#path-effect299"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g><g
         id="g120"
         inkscape:label="single genus "
         style="display:inline;stroke-width:1.805;stroke-dasharray:none"
         transform="matrix(0.7710386,0,0,0.7809002,-81.12324,370.19338)"><path
           style="display:inline;fill:url(#radialGradient125);fill-opacity:1;stroke:none;stroke-width:1.8288;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path116"
           inkscape:label="shadowR"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath218)" /><path
           style="display:inline;fill:url(#radialGradient126);fill-opacity:1;stroke:none;stroke-width:1.8288;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path117"
           inkscape:label="shadowL purp"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath217)" /><g
           id="g119"
           inkscape:label="genus hole 1"
           style="display:inline;stroke-width:1.8288;stroke-dasharray:none"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.8288;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path118"
             inkscape:path-effect="#path-effect121"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             transform="translate(311.23778,-33.331065)"
             sodipodi:nodetypes="cscc" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.8288;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path119"
             inkscape:path-effect="#path-effect123"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g><g
         id="g197"
         inkscape:label="Curves"
         transform="matrix(1.0563381,0,0,1.0611073,-393.9397,104.64762)"
         style="display:inline;stroke-width:1.32292;stroke-dasharray:none"><path
           style="fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
           d="m 991.37834,463.5468 c -18.17372,-14.38731 -65.09288,-20.14053 -97.97009,1.31812"
           id="path193"
           sodipodi:nodetypes="cc"
           inkscape:transform-center-x="2.1983096"
           inkscape:transform-center-y="1.5044513" /></g><path
         style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.805;stroke-dasharray:none;stroke-opacity:1"
         d="m 398.9881,575.37435 c -34.28156,0.65578 -67.99587,-7.67395 -101.74254,-13.74168 -33.74667,-6.06773 -69.00063,-9.82682 -101.92467,-0.25276 -18.64174,5.42087 -36.21443,15.2148 -49.46431,29.40427 -13.24988,14.18948 -21.94997,32.91493 -22.64256,52.31649 -0.79494,22.26858 9.08456,44.29902 24.86282,60.0333 15.77827,15.73429 37.04462,25.3906 59.02738,29.03474 32.26538,5.34871 65.20665,-1.70763 96.87054,-9.89675 31.66388,-8.18911 63.58289,-17.6241 96.28417,-17.08584 35.0282,0.57656 68.69437,12.54539 102.45677,21.89456 33.76241,9.34916 69.87692,16.13073 103.52586,6.38106 19.76739,-5.72754 37.96575,-17.23521 50.88264,-33.25734 12.91689,-16.02212 20.35093,-36.57578 19.73059,-57.14687 -0.55924,-18.54504 -7.60848,-36.70135 -19.03896,-51.31556 -11.43049,-14.6142 -27.11202,-25.71598 -44.39244,-32.47011 -33.8066,-13.21347 -71.7641,-9.71219 -107.34058,-2.51524 -35.57649,7.19694 -70.80421,17.92352 -107.09471,18.61773 z"
         id="path46"
         inkscape:path-effect="#path-effect109"
         inkscape:original-d="m 398.9881,575.37435 c -66.26804,27.41298 -72.61511,-32.04957 -203.66721,-13.99444 -84.32861,11.61801 -72.88663,142.18816 -72.10687,81.72076 0.69433,-53.84253 32.36522,76.07526 83.8902,89.06804 46.98614,11.84825 151.41593,-27.71058 193.15471,-26.98259 81.2214,1.41662 124.13592,34.84951 205.98263,28.27562 24.94759,-2.00379 52.96994,-72.26893 70.61323,-90.40421 21.40106,-21.99789 -33.72152,-79.09133 -63.4314,-83.78567 -62.8792,-9.9353 -130.40936,-23.10067 -214.43529,16.10249 z"
         sodipodi:nodetypes="csssssssc"
         inkscape:label="surface"
         transform="matrix(0.77103859,0,0,0.78090021,131.2251,94.533162)" /></g><g
       id="g94"
       inkscape:label="mapArrow"
       transform="matrix(0.94666662,0,0,0.94241181,620.11761,-65.711746)"
       style="display:inline"><path
         style="display:none;opacity:1;fill:none;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-dashoffset:0;stroke-opacity:1"
         d="M 435.70117,454.97998 Z"
         id="path93" /><path
         style="display:inline;opacity:1;fill:none;stroke:#000000;stroke-width:1.4006;stroke-linejoin:round;stroke-dasharray:none;stroke-dashoffset:0;stroke-opacity:1;marker-start:url(#ArrowWideRounded);marker-mid:url(#Triangle);paint-order:stroke fill markers"
         d="m 450.05787,470.70709 c 0.2586,-23.7014 0.003,-84.6503 0.003,-84.6503"
         id="path94"
         inkscape:label="tail"
         sodipodi:nodetypes="cc" /></g><g
       id="g126"
       inkscape:label="genus and curve"><g
         id="g201"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient201);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path200"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient202);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path205"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient209);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path201"
           inkscape:label="shadowR"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath218)" /><path
           style="display:inline;fill:url(#radialGradient211);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path211"
           inkscape:label="shadowL purp"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath217)" /><g
           id="g60"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path59"
             inkscape:path-effect="#path-effect68"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             transform="translate(311.23778,-33.331065)"
             sodipodi:nodetypes="cscc" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path60"
             inkscape:path-effect="#path-effect70"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g><g
         id="g342"
         inkscape:label="Curves"
         transform="translate(118.75748,-0.25705083)"><path
           style="fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:0.926042;stroke-dasharray:none;stroke-opacity:1"
           d="m 860.39634,137.30588 c -14.28419,18.25487 -21.28094,87.57152 0.36351,120.32671"
           id="path341"
           sodipodi:nodetypes="cc" /><path
           style="opacity:0.512626;fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:0.926042;stroke-dasharray:11.1125, 11.1125;stroke-dashoffset:0;stroke-opacity:1"
           d="m 861.63439,138.0363 10e-6,118.75748"
           id="path342"
           sodipodi:nodetypes="cc" /></g></g><g
       id="g147"
       inkscape:label="genus and curve"
       transform="translate(146.50048)"><g
         id="g145"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient150);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path139"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient151);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path140"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient151);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path141"
           inkscape:label="shadowR"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath218)" /><path
           style="display:inline;fill:url(#radialGradient152);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path142"
           inkscape:label="shadowL purp"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath217)" /><g
           id="g144"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path143"
             inkscape:path-effect="#path-effect148"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             transform="translate(311.23778,-33.331065)"
             sodipodi:nodetypes="cscc" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path144"
             inkscape:path-effect="#path-effect150"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g><g
         id="g146"
         inkscape:label="Curves"
         transform="translate(118.75748,-0.25705083)"><path
           style="fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:0.926042;stroke-dasharray:none;stroke-opacity:1"
           d="m 860.39634,137.30588 c -14.28419,18.25487 -21.28094,87.57152 0.36351,120.32671"
           id="path145"
           sodipodi:nodetypes="cc" /><path
           style="opacity:0.512626;fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:0.926042;stroke-dasharray:11.1125, 11.1125;stroke-dashoffset:0;stroke-opacity:1"
           d="m 861.63439,138.0363 10e-6,118.75748"
           id="path146"
           sodipodi:nodetypes="cc" /></g></g><g
       id="g160"
       inkscape:label="genus and curve"
       transform="translate(-144.99516)"><g
         id="g158"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient163);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path152"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient164);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path153"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient164);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path154"
           inkscape:label="shadowR"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath218)" /><path
           style="display:inline;fill:url(#radialGradient165);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path155"
           inkscape:label="shadowL purp"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath217)" /><g
           id="g157"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path156"
             inkscape:path-effect="#path-effect161"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             transform="translate(311.23778,-33.331065)"
             sodipodi:nodetypes="cscc" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path157"
             inkscape:path-effect="#path-effect163"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g><g
         id="g159"
         inkscape:label="Curves"
         transform="translate(118.75748,-0.25705083)"><path
           style="fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:0.926042;stroke-dasharray:none;stroke-opacity:1"
           d="m 860.39634,137.30588 c -14.28419,18.25487 -21.28094,87.57152 0.36351,120.32671"
           id="path158"
           sodipodi:nodetypes="cc" /><path
           style="opacity:0.512626;fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:0.926042;stroke-dasharray:11.1125, 11.1125;stroke-dashoffset:0;stroke-opacity:1"
           d="m 861.12029,137.26515 c 0.58077,51.43899 0.47796,50.46123 -0.21294,120.25568"
           id="path159"
           sodipodi:nodetypes="cc" /></g></g><g
       id="g173"
       inkscape:label="genus and curve"
       transform="translate(291.59808,-0.72704953)"><g
         id="g171"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient176);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path165"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient177);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path166"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient177);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path167"
           inkscape:label="shadowR"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath218)" /><path
           style="display:inline;fill:url(#radialGradient178);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path168"
           inkscape:label="shadowL purp"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath217)" /><g
           id="g170"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path169"
             inkscape:path-effect="#path-effect174"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             transform="translate(311.23778,-33.331065)"
             sodipodi:nodetypes="cscc" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path170"
             inkscape:path-effect="#path-effect176"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g><g
         id="g172"
         inkscape:label="Curves"
         transform="translate(118.75748,-0.25705083)"><path
           style="fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:0.926042;stroke-dasharray:none;stroke-opacity:1"
           d="m 860.39634,137.30588 c -14.28419,18.25487 -21.28094,87.57152 0.36351,120.32671"
           id="path171"
           sodipodi:nodetypes="cc" /><path
           style="opacity:0.512626;fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:0.926042;stroke-dasharray:11.1125, 11.1125;stroke-dashoffset:0;stroke-opacity:1"
           d="m 862.94849,136.74557 c -0.455,23.28631 -1.25368,99.52416 -1.24114,120.76977"
           id="path159-5"
           sodipodi:nodetypes="cc" /></g></g><g
       id="g186"
       inkscape:label="genus and curve"
       transform="translate(-290.74719,-0.08063906)"
       style="display:inline"><g
         id="g184"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient191);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path178"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient192);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path179"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient192);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path180"
           inkscape:label="shadowR"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath218)" /><path
           style="display:inline;fill:url(#radialGradient193);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path181"
           inkscape:label="shadowL purp"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)"
           clip-path="url(#clipPath217)" /><g
           id="g183"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path182"
             inkscape:path-effect="#path-effect187"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             transform="translate(311.23778,-33.331065)"
             sodipodi:nodetypes="cscc" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path183"
             inkscape:path-effect="#path-effect189"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g></g><text
       xml:space="preserve"
       transform="scale(0.26458333)"
       id="text197"
       style="white-space:pre;shape-inside:url(#rect197);display:inline;opacity:0.512626;fill:#1a1a1a;stroke:#000000;stroke-width:3.5;stroke-dasharray:42, 42;stroke-dashoffset:0" /><text
       xml:space="preserve"
       transform="scale(0.26458333)"
       id="text198"
       style="white-space:pre;shape-inside:url(#rect198);display:inline;opacity:0.512626;fill:#1a1a1a;stroke:#000000;stroke-width:3.5;stroke-dasharray:42, 42;stroke-dashoffset:0" /><image
       width="45.772915"
       height="38.893749"
       preserveAspectRatio="none"
       xlink:href="data:image/png;base64,iVBORw0KGgoAAAANSUhEUgAAAK0AAACTCAYAAAD835meAAAABHNCSVQICAgIfAhkiAAADA9JREFU&#10;eJzt3XtsFFUbBvCnlJYKS6mkjUWkfBSRq8pFEKzWclGMCIIXlGCQaAQhAbzEgEYFDQrEqEGr0ZCA&#10;GAGbQuRmg8pNkYsoghpEsECAQqHcaim0UNjz/fFmM91e6G47szvv8PySpu6Unpk1T8+emXnPmRhj&#10;jAGRIo2ifQBE4WJoSR2GltRhaEkdhpbUYWhJHYaW1GFoSR2GltRhaEkdhpbUYWhJHYaW1GFoSR2G&#10;ltRhaEkdhpbUYWhJHYaW1GFoSR2GltRhaEkdhpbUYWhJHYaW1GFoSR2GltRhaEkdhpbUYWhJHYaW&#10;1Lk2Qnv+PBDJZXi55K+jvBfaK1eAH34Ann0W6NMHaNkS8PmAhAQgPR14+mkgNxeoqHBm/3v3Aj17&#10;yjGQM4xXlJQYM2OGMampxkhfd/Wvtm2NmTfPmIoK+45h8WJjfD5pf9o0+9qlIPpD6/cb88knxqSk&#10;hBbWql/t2hkzf74xly/X/xgKCowZNUrai4+XPwZyTIwxigdgR44AY8cC69db2xITgawsoEMHoH17&#10;ICkJOHYMyM8H8vKAw4drbqtjR+Dtt4HHHwdiYkLb/8WLwIcfAjNnyrg5NRVYtgy4666GvjO6mmj/&#10;1dTbmjXGXH+91WNmZhqzcKEx589f/fe2bDFm8ODae97u3Y3JzTXmwoXa2/jjD2NeeMGY5GTr9+68&#10;U3pccpzOnvb994GpU+Wkq1s3YO5cYMCA8NrYtAl4/XXgp59q/nnTpkBmJvC//0kPeuqU9Nb79gEH&#10;Dlj/rnFj4LXXgDfekP8m50X7ryYsZWXGjB4tPZvPZ8zcuQ0/kfruO+kl6zMezsoyZscOe94bhUxX&#10;aAMf6127GrNnj71tf/utMb161R3U2Fg5jrw8e/dPIdM1PFi/Hli0CPj4Y/n4dsIvvwCrVwPbtskJ&#10;3LlzQNu2clLXowfwxBMyXKCo0RVaInjxjhh5HkNL6jC0pA5DS+owtKQOQ0vqMLSkDkNL6jC0pA5D&#10;S+owtKQOQ0vqXNtVy2VlUgy+dq1Mwzl9GjhzRqbstGoF9OoFDB0K3HJLtI+UKrk2q7xOnADmzAE+&#10;+0yCW5f+/YH33pMQU9RdW8MDY6QWNz1dJiT6fDJVZt06qZ0tLwcOHZI1C+bOlRpaANiwAejdG5g9&#10;O7rHTyKaFegRVVRkzIABMvsgJcWYOXOMKS29+u+Ulxvz7rsyLTwwc2HKlMgcL9Xq2gjt33/L+gaA&#10;TJUpLg7v92fODJ5ys2CBI4dJofH+mHb/fiAjQ8axEybI8CA2Nrw2KiqAO+4A/vxTXicmAgcPypJL&#10;FHHeHtOeOgXcf78Edvp04NNPww8sAMTFAa+8Yr0uKZFp7BQV3u5pR4wAli8HnnwSWLKkYW0dOiRr&#10;IASkpck2ijjvhnbBAuCZZ+Qy1aZNwHXXNay9S5eAJk2Ct+3eDXTp0rB2KWzeHB4cPAhMmSLTzHNz&#10;Gx5YQIYIjar87/rnn4a3S2Hz3h0xvx8YM0bWK5gzB2jXzp52S0qk7coKC+1pm8LivZ42Jwf4+WdZ&#10;4+ull+xrt6aAhrq6ItnKW6H1+2W5TkDuaNm5INyuXdW3tWplX/sUMm+FdvFiGWdmZIS/imJdNm2q&#10;vq1bN3v3QSHxztWDK1eAzp2Bf/8F1qwBBg+2r+2LF4Ebb5QKsID27WXpT4o47/S0S5ZIYHv2tDew&#10;ALBiRXBgAWD0aHv3QSHzTmi/+EK+jxtnf9vz5we/btYMmDzZ/v1QSLwxPCgqko/vJk3kLD8x0b62&#10;t28H+vULvtw1axYwbZp9+6CweKOnzc2VMe2jj9ob2LIyee5Y5cD27h1ch0AR543Q5uTI9xEj7G33&#10;1VeD73p16ACsWlW/ohuyjf7hQVGRrMwdFydzvHw+e9pdvRoYNsx6ZGhamlz2Skuzp32qN/23cTdu&#10;lGBlZoYW2NJSqY9NSKi9JmHlSmDkSCuwqaky+ZGBdQVvhBao/WZCUZFMYMzNlUKa8+etnzVuDLRo&#10;AXTtCgwcKG2sWiWTGAOBffBBuXpwww2Ovg0Knf7hQZcuwJ49wNatQN++wT87dw7o1EkmLfp8cvMh&#10;MVFqBvx+OdHavVuKYapq2lTCO3FiZN4HhUx3T3vihATW55PpMFXt2SOBBYCnnpIhRGBIcOkScPy4&#10;9NQrV8rVh8oyMuRJ5uQ+0ZiYZpucHJlo+MADNf+8vNyYhx4yJiam7ueDde9uzNSpwTNvMzONOXs2&#10;su+J6qS7pw2MZ/v3r/nnTZrIGPXwYWDHDhnfVlTI8CA2Vu5spaYC3bsDKSnyO127Sj0uII8gffhh&#10;WfegagE4RY3uMW3nznIddft2uehvl5dfBj74wHrNO2Cuoje0x49LPWtiohSz2HnB/8wZmcR47py8&#10;josDfv0VuP12+/ZB9ab3M+/HH+X7PffYf4eqZUtg/HjrdUUFp4zXZMUKIC8v4rvVG9q6xrMNNXBg&#10;8OulS4HiYmf2pU15udRkDB8ODBki5woRxNDWpk+f4NdlZcBXXzmzLy38fqlb7tED+PJLa3tgGBUh&#10;Ose0gfFsUpLUGzh1Zt+sGXDhgvX6vvuA7793Zl9uVVoKbN4sncSyZVJoX1V+vrXCZATovOQVGM9m&#10;Zjp7KSopKTi0O3c6ty+3WLpUxu9nzgBnz0qnECjNTEgAOnYE9u6N6iHqHB5s2CDfnRoaBFQtqDl1&#10;KjjEXnToELBtG7BvH3DyJNC2rRQPzZsnn3CTJkX7CJX2tE6PZwNqOvE6e1bqErxqzBiZY5eYKEVC&#10;VZeCcgF9oT1+XD6eWrYEbrvN2X3VFNr4eGf3GW0pKdbdQZfSNzwI9LL33uvsCi8lJdWLaOLjgeRk&#10;5/ZJIdEbWqeHBjWdbNx0E5dCcgGGtjZbt1bf1rq1s/ukkOgKbWGh9IDJyVKN5aQtW6pv4zJIrqAr&#10;tIFe9u67nf+Y3ry5+rbHHnN2nxQSnaF1+qrBli1AQUHwtpQUOfmjqNMZ2ptvdnY/CxdW3/bII1zv&#10;wCX0hLawUO7SAFIT4JTycmvxj4DYWE5wdBE9oQ30soAEyynz5wP//Re8bdw454ckFDKdoT192pl9&#10;lJQAM2YEb0tKslYXJ1fQGVqnnirzzjtSJFLZrFm8C+YyOkJ77Jg1ngVqvobaUMuXV59SM2EC8Pzz&#10;9u+LGkRHaAO9bL9+QPPm8tAOO2s6N26UpzpWrjUYMkSeo0uuoyu0w4dbEw4/+sietn/7TVZHvHjR&#10;2paRAXz9NS9xuZSu0A4YALz4olRbff65TOuuL2Mk+JmZwXOcxo8H1q+3b8lQsp3762mPHZN5SS1a&#10;yIS62FhZ7Pitt+S26oYNQHp6eG0WFABjxwLr1lnb4uOB7GzguecadrzffCOPhjpxwlp5MVri4mTm&#10;wfTpwQ+j1i6aazKFZNEiWVdr6NDg7RMnyvbWrY3Jywutrd27jZk0yZjmza31umJijBk50ph9++w5&#10;3s6d6143LNJfb75pz3szxpjs7Ort5+fb134I3N/T1laKmJ0ti2jMmydryA4aBIwaBWRlyUNDEhJk&#10;Pld+vsx5WrIk+LIZILNrZ8+WxzjZZfJkeQL6yZPu6GnbtJFnUXhJRP9E6qNDB/lr3rmz5p/v2GHM&#10;sGHV//orr35Y+at3b2NmzTJm797Ivg+vYE9bh6NHZTx7tflgPXvK8jx//SVrEvz+u/RypaVSmdWm&#10;jcw4SEuTkkYuQa+eu0NbeT5YXesb3HqrfJHnufuSV6Sm1pAqDC2p497QHj0qZ/4pKc7PByNV3Bva&#10;QC+blcVp2xTE/aHl0ICqcG9oI7XIHIXn0qXQtjnInaEtKAD275cnz3TqFO2jocoOHKi+7eDBiB6C&#10;O6/TcmjgLn6/dCR5efLI1qoCy3/27Ss3ghzG0FKwwkKrFsPvl4/+khJrYeWaHDggRfOAVMs1by7V&#10;eI0ayZWftWttPUSGloL5/bIKuM9nPak9OdkKYUxM9as5xsjv+f3A5ctSyFRRIQVLDjxcxX3PXCgo&#10;sOoFjhyJ9tGQC7nvRIy9LNXBfaHdtUu+M7RUC/cND4qLZYr4oEHeXyqe6sV9oSWqg/uGB0R1YGhJ&#10;HYaW1GFoSR2GltRhaEkdhpbUYWhJHYaW1GFoSR2GltRhaEkdhpbUYWhJHYaW1GFoSR2GltRhaEkd&#10;hpbU+T/enpHgxNYeVwAAAABJRU5ErkJggg==&#10;"
       id="image1"
       x="808.85822"
       y="263.3754" /><image
       width="51.329166"
       height="49.741665"
       preserveAspectRatio="none"
       xlink:href="data:image/png;base64,iVBORw0KGgoAAAANSUhEUgAAAMIAAAC8CAYAAAAqyXGAAAAABHNCSVQICAgIfAhkiAAADwJJREFU&#10;eJzt3XlwF+Udx/E3iQSFGAIlGvBAQEXBA1G8kIgHYr0RtVo6tmrrNY54jsfoiI4FGW0ZVByVEeuM&#10;ghgPKqh4oRVFRXHQihQVNRgJRkQMN4E8/ePb7e/aX/I7dhN+7Oc1w8TdZJ/djPn89nmefZ5n2znn&#10;HCIRV9TWFyCyLVAQRFAQRAAFQQRQEEQABUEEUBBEAAVBBFAQRAAFQQRQEEQABUEEUBBEAAVBBFAQ&#10;RAAFQQRQEEQABUEEUBBEAAVBBFAQRAAFQQRQEEQABUEEUBBEAAVBBFAQRAAFQQRQEEQABUEEUBBE&#10;AAVBBFAQRAAFQQRQEEQABUEEUBBEAAUheOvWQWu+qFQvRQ2EgpCPrVvh9dfhkkvg8MOha1coLYUd&#10;d4TeveGPf4TqamhsDOf8S5bAwIF2DZIfJ9lraHBuzBjnKiuds8/k5v/17Onc5MnONTYGdw1TpzpX&#10;Wmrl33xzcOVGlIKQjaYm5yZNcq6iIrMAJP/r1cu5KVOc27Il92uorXXuggusvJISC5jkrZ1zqmRm&#10;5Pvv4U9/gjlzYvvKymDoUNhnH+jTB8rLYfly+PprePllWLbMv6y+feGuu+Dcc6Fdu8zOv2kTTJgA&#10;d99t7ZDKSnjuOTj66Hx/MwFVjTIye7ZzXbrEPtmrqpx74gnn1q1r/rh585wbPjz9HWLAAOeqq51b&#10;vz59GZ9+6tw11zjXrVvsuCOOsDuDBEZ3hJb87W9w003WMD7gAJg4EY4/Prsy5s6F226Dd97x/37H&#10;jlBVBXvtZZ/0K1faXeXLL+Gbb2I/t8MOcOutcPvt9t8SnLZO4jZrwwbnRo2yT+DSUucmTsy/sfvq&#10;q/Zpnkv7YuhQ5xYsCOZ3kxQKQjpelaZ/f+cWLw627Jdecu7QQ1v+4y8utut4+eVgzy8pVDVKZ84c&#10;eOopeOABq7qE4cMPYdYs+OADa2SvWQM9e1rD+5BD4He/s6qShE5BEEFPlkUABUEEUBBEAAVBBFAQ&#10;RAAFQQRQEEQABUEEUBBEAAVBBFAQRAAFQQQAze5oLRs22ASdN96wKZw//wyrVtl0z+7d4dBD4fTT&#10;Yd992/pKI0mjT8P2448wfjw8/LCFoSXHHQf33mvBkFajqlFYnLO5DL1726T70lKbZvnmmzb3YONG&#10;qKmxNYkmTrQ5CABvvQWDBsE997Tt9UdNW84K2m7V1zt3/PE2y6yiwrnx451bu7b5YzZudG7sWFui&#10;xZuhNnp061yvaKpm4L74wtYvAptmuXp1dsfffXfidM3HHw/lMiWR2ghBWroUBg+2dsEVV1jVqLg4&#10;uzIaG+Gww+Czz2y7rAy+/daWk5TQqI0QlJUr4aSTLAR33AEPPZR9CADat4cbb4xtNzTYkjISKt0R&#10;gjJiBMyYAeefD9Om5VdWTY2tceTZc0/bJ6FREILw+ONw8cXW5Tl3Luy0U37lbd4MHTok7lu0CPr1&#10;y69cSUtVo3x9+y2MHm1LvlRX5x8CsOpRUdL/mv/8J/9yJS09Wc5HUxNceKGtRzR+PPTqFUy5DQ1W&#10;dry6umDKFl+6I+Rj+nR4911bE/W664Ir1++PPtNVsyUnCkKumppsaXewJ8NBLsq7cGHqvu7dgytf&#10;UigIuZo61ertgwdnvzp2S+bOTd13wAHBnkMSqNcoF1u3wv77w1dfwezZMHx4cGVv2gQ9etjIVE+f&#10;PrZMvIRGd4RcTJtmIRg4MNgQAPzzn4khABg1KthzSAoFIRf/+Id9vfTS4MueMiVxu1MnuPrq4M8j&#10;CVQ1ylZ9vVVdOnSw3p2ysuDKnj8fjjoqset03Di4+ebgziG+dEfIVnW1tRFGjgw2BBs22HuZ40Mw&#10;aFDiuCMJjYKQrenT7euIEcGWe8stiU+P99kHZs7MbeCeZE1Vo2zU19sbbNq3tznHpaXBlDtrFpxx&#10;hs1AABtkN3eufZVWoSEW2Xj7bftjrarKLARr19r8gh13TD8G6cUX4bzzYiGorLQJ/gpBq1IQsvH2&#10;2/Y13QO0+nqbpF9dbYPx1q2LfW+HHaBzZ+jfH044wcqYOdMm6nshOOUU6zXadddQfw1JpapRNvr1&#10;g8WL4f334cgjE7+3Zg3st59NzC8ttQduZWU2RqipyRrDixbZgLpkHTtaIK68snV+D0mhO0KmfvzR&#10;QlBaalMpky1ebCEA+MMfrPrkVYc2b4YVK+yO8uKL1usUb/BguOSSUC9fWtAWE6UL0vTpNpn+5JP9&#10;v79xo3OnneZcu3Ytvz95wADnbropccWKqirnfvmldX8n+T/dETLltQ+OO87/+x06WJ1/2TJYsMDa&#10;C42NVjUqLrYnxJWVMGAAVFTYMf3723wGgHfegTPPtHWNkiflSOjURsjU/vtbP//8+fagKyjXXw9/&#10;/3tsW0+S24SCkIkVK2w+QFmZDYgL8iHXqlU2UX/NGttu3x4++ggOPji4c0iLdA/OxL/+ZV+HDAn+&#10;SW/XrnDZZbHtxsZglm/56Sd47z147jkbJPjqq/D556kNdQHUa5SZltoH+TrhBLjvvtj2s8/C/fdD&#10;eXl25WzaBI88YsPE589PnfcMsMsu9gBv1KjULuAIU9UoE177YMECm4MQtFWr4De/Sdz3wANw1VWZ&#10;l/HKK3Zn+f572+7VK7bETHm5rYv05pvw5JO2ADHAWWfBpEk2mjbq2rLLqiDU1Vn3Znm5c1u3hnee&#10;jh0Tu1iHDcv82Hvvda6oyI7r3Nm5qVOda2ry/9n6eucuuih2nt12c+6TT4L5HQqYgtCSp5+2P5gz&#10;zgj3PD16JAahW7fMjps0KXZMp07OffxxZsfdeGPsuIoK55Yuzf3atwNqLLfkrbfsa1jtA0/yoLyV&#10;K2H9+uaP+egjuOaa2PaECZm/YOSee2wSEFjDeuTISDekFYSWhN1Q9qxenbrvl1/S//zWrfDnP1sv&#10;E0DfvtYmyFRREYwdG9teuBAefDDz47czCkJzVqyAJUusi/Ogg8I9l18QSkrS//y0abGl4wF+//vs&#10;u3aHDoU99ohtjx1rPU8RpCA0x7sbHHtsuCvNNTSkVktKSqBbt/THTJ6cuH3qqbmd+7e/jf13fT08&#10;80xu5RQ4BaE5rVUtWrIkdd/uu6cPX01N4iJgRUW5LwCWfFxEq0cKQnNaKwjvv5+6b7fd0v/8U0/F&#10;JvOAVW+Sl5HP1H77JW7Pn29VwohRENKpq7NP6m7dbJRomObNS93X3Cf8a68lbuczrdPvWO8DIEIU&#10;hHS8P4Zjjgl/Jer33kvdd8456X/+008Tt/N5v1ryE22AOXNyL69AKQjpeEEIu7do3jyorU3cV1Fh&#10;DXQ/NTWpPUxduuR+/i5dUoO+aFHu5RUoBSEdLwh77x3ueZ54InXf2Wen7wqN7zL1dOyY+/mLi1O7&#10;aSP4vjYFwU9dHXz5pf13p07hnWfjxtiCYZ7i4uYn8fu9RCTfoeHJ73aoq4s9qIsIBcFPfGPRG6kZ&#10;hilT4NdfE/ddemnz1bGVK1P35fuSkuQgNTVFrudIQfATH4Sffw7nHA0NMGZM4r7y8thbeNL56afU&#10;fUHfEcCWn4kQBcFPfBDCepvlX/+a+kc9blzzT5MhcdEwT753BL/jw7wTboMUhGTLl8faB+Dfx5+v&#10;GTNSp2NecQVcfnnLx/rV3cO4IygIEefdDY46Cnbe2UZl+g2ByKf8889PHFt06qk2Iy0TfkOlw3jO&#10;EbHBdwpCMi8IZ50Vm1R///3BlP3xx7bqdfwf2eDB8PTTmX+q+3165zvb1u/4iC1HryAki1/o99pr&#10;rY/9kUdsEkyunLMwVVXFlm0BC9qcOdktL9++feo+v0n62V5fJufZjikI8ZYvt5cEdu4Mhxxik9pv&#10;ucWqI+ecA998k32ZtbUwbBiMHh3riSkpgUcftZWzm5tz4Mfv57dsyf664vm1O7K9rgKnIMTz7gZV&#10;VbGqwZgx9oBr2TLb/8ormZX1xRf2EsB+/Wz1CLC6/Hnn2fpCf/lLbtfo16u0eXNuZTV3fEu9V9sZ&#10;rWsUL92w6wcftE/NyZPtHQYnnggXXGAzvHr0sBeBrF9v70L+4AObPZY8gnPYMJsnnO9yMH5Lr+Tb&#10;sPU7fpdd8iuzwCgI8dIFoV07q8pcfjnceact7f7GG7Hvl5T4f6oOGmTjhs4+G/bdN5hr7N49dV98&#10;uyNbmzenXnuXLpFrIygInh9+sPZBc/OTBw60F4L/+982J+CTT+yh2Nq1NmJ0jz1sZtmee9rw7TBe&#10;/7TXXqn7kodpZMNvgYC+fXMvr0ApCJ74+cktLct+4IH2ry3062eLEce/eSfoIPi9CGU7p8ayp7Wm&#10;ZearqAiOPjpx3w8/5F6e37EKQoQVShDAql3xli3LfXGu+OEkniFDciurgCkIYJ+KX39t9fyw5ycH&#10;4fTTE7e3bIHvvsutrORBhVVV0Lt3bmUVMAUBYneDoUPDn58chIMOsi7ceLlOuPfe/eCJ6EsNFQQo&#10;rGqR54YbErdnzcq+jOXLExcC6Nq1+UUDtmMKArTeQr9BGj48sedq5kxYujS7MpIHE44bl9/85wKm&#10;F4XU1lr/f2Wl/3zgbdmHH1rD2RtrNGIEPP98Zsd+951VsbyHcUOG2J0xom/0jOZvHa8Qq0WeI45I&#10;nMfwwgs2860lv/5qVSAvBH36WIAiGgJQEAo7CGDDPh57LLbaxm232fLwfpP8AWbPtklHCxbY9sCB&#10;VjWM2CC7ZKoa7b231a2/+ir8NYzCVFNj0z290bE77WQrXffvb2OHamttWMjnn9v3S0psvsUdd6S+&#10;pCSCoh0Er32w++6xl/AVunfftVfKzpiR+myhuNieE4wcaf8qK9vkErdF0R5rVOjVIj/HHGP/Jkyw&#10;FS/q6qwtUFEBu+4auVGlmYp2EBYutK/bUxDidepU2NW9VhTtqtHq1bZcy4knRm5qoiSKdhBE/kfd&#10;pyIoCCKAgiACKAgigIIgAigIIoCCIAIoCCKAgiACKAgigIIgAigIIoCCIAIoCCKAgiACKAgigIIg&#10;AigIIoCCIAIoCCKAgiACKAgigIIgAigIIoCCIAIoCCKAgiACKAgigIIgAigIIoCCIAIoCCKAgiAC&#10;KAgigIIgAigIIoCCIAIoCCKAgiACKAgigIIgAigIIoCCIAIoCCKAgiACKAgigIIgAigIIoCCIAIo&#10;CCKAgiACKAgigIIgAigIIgD8Fz981vTS51qmAAAAAElFTkSuQmCC&#10;"
       id="image1-0"
       x="950.76288"
       y="260.13257" /><image
       width="41.274998"
       height="43.127083"
       preserveAspectRatio="none"
       xlink:href="data:image/png;base64,iVBORw0KGgoAAAANSUhEUgAAAJwAAACjCAYAAAB/lHc1AAAABHNCSVQICAgIfAhkiAAAC+NJREFU&#10;eJztnXtsFFUUh3+l0FZYSm26saAWASsVUHlYBKtreShGFMEHSjBoNIKYKEpiQKORGBSIMQZFozYp&#10;YpRKCgkvERUBRUBRBB+AYGlTKLRUHnVbaKGw1z9O1ul2ty925m5n5vclTd1Z9s6s+Xofc885E6eU&#10;UiBEEx1ifQHEXVA4ohUKR7RC4YhWKBzRCoUjWqFwRCsUjmiFwhGtUDiiFQpHtELhiFYoHNEKhSNa&#10;oXBEKxSOaIXCEa1QOKIVCke0QuGIVigc0QqFI1qhcEQrFI5ohcIRrVA4ohUKR7RC4YhWKBzRCoWL&#10;xOnTgM6iUi4qYEXhLlwAvvkGeOIJYOhQIDUV8HiApCSgd2/g0UeBwkKgvt6a8+/fDwweLNfgBpRb&#10;8fuVmjNHqfR0paSPaf6nZ0+l8vKUqq837xqWLlXK45H2Z882r912jPuECwSUeu89pbze1onW+KdX&#10;L6Xy85U6f/7ir6GsTKlJk6S9hAQR2SXEKeWiCcThw8BjjwEbNxrHkpOB3FwgMxPo0wdISQGOHgWK&#10;ioB164BDhyK31bcv8NprwIMPAnFxrTv/2bPA228Dc+fKPDE9HVixArj55mi/mX2ItfHaWL9eqUsv&#10;NXoqn0+pJUuUOn26+c9t26bUmDFN93gDBypVWKjUmTNNt/Hbb0o995xSaWnG5266SXo6l+GOHu6t&#10;t4BZs2SBMGAAsHAhMHJk29rYsgV4+WXg++8jv9+5M+DzAVddJT3X8ePSSx44ABQXG/+uY0fgpZeA&#10;V16R/3YbsTbeUmprlZo8WXoUj0ephQujn/R/9ZX0Thcz/8vNVWrnTnO+m01xtnDBobB/f6X27TO3&#10;7S++UGrIkJYli4+X61i3ztzz2xRnD6kbNwKffQa8+64MeVbw00/A2rXAjz/KYqO6GujZUxYggwYB&#10;Dz0kQywBADhbONLu4E4D0QqFI1qhcEQrFI5ohcIRrVA4ohUKR7RC4YhWKBzRCoUjWqFwRCsUjmjF&#10;hRGAF0ltrQRhbtggYecnTgAnT0qIevfuwJAhwD33ANdcE+srbdcwWqQljh0DFiwAPvhApGuJESOA&#10;N98UAUkYHFKbQimJo+vdWxJfPB4JDf/2W4l7q6sDSksln3ThQol/A4BNm4DsbGD+/Nhef3slltGf&#10;7ZbKSqVGjpSIXa9XqQULlKqpaf4zdXVKvfGGpP0Fo31nzNBzvTaCwjVm717JPQUkNLyqqm2fnzs3&#10;NMR88WJLLtOucA7XkIMHgZwcmbdNny5Danx829qorwduvBH4/Xd5nZwMlJRICQnCOdz/HD8O3HGH&#10;yPbqq8D777ddNgDo1Al44QXjtd8vaYoEAFepBhMmACtXAg8/DBQURNdWaankpwbJyJBjhMIBABYv&#10;Bh5/XG5lbNkCXHJJdO2dOwckJoYe27MH6NcvunYdAIfUkhJgxgxJIywsjF42QIbVDo3+1/71V/Tt&#10;OgB37zQEAsCUKZJLumAB0KuXOe36/dJ2Q8rLzWnb5ri7h1u2DPjhB6k3MnOmee1Gkqu1FZYcjnuF&#10;CwSk3BYgOwVmFpbZvTv8WPfu5rVvY9wr3NKlMq/KyWl7JaWW2LIl/NiAAeaew6a4c5V64QJw7bXA&#10;338D69cDY8aY1/bZs0CPHhJJEqRPHyndRVzawxUUiGyDB5srGwCsWhUqGwBMnmzuOWyMO4X7+GP5&#10;PXWq+W3n54e+7tIFePZZ889jU9w3pFZWypCXmCiryeRk89resQMYPjz0lsi8ecDs2eadw+a4r4cr&#10;LJQ53P33mytbba0806GhbNnZofuqxIXCLVsmvydMMLfdF18M3U3IzATWrLm4AAAH464htbJSqlF2&#10;6iQ5CR6POe2uXQuMG2c8wigjQ26NZGSY076DcNfW1ubNIoXP1zrZamokvi0pqek91tWrgYkTDdnS&#10;0yXRhrJFxH3CAU3f6K2slGSZwkLZ1D992nivY0egWzegf39g1ChpY80aSZgJynbXXbJKvewyS7+G&#10;nXHXkNqvH7BvH7B9OzBsWOh71dVAVpYkyHg8cmM4OVn2QAMBWRTs2SMb843p3FnEe/ppPd/Dxrin&#10;hzt2TGTzeCQEvDH79olsAPDIIzLsBofRc+eAigrpIVevllVuQ3Jy5GmEpGVikUgRE5Ytk6SWO++M&#10;/H5dnVJ3361UXFzLz14YOFCpWbNCM7R8PqVOndL7nWyIe3q44PxtxIjI7ycmypzs0CFg506Zz9XX&#10;y5AaHy87BunpwMCBgNcrn+nfX+LpAHkk0r33Sl5q4+BLYhBr47WRlSU90Y4d5rY7c2Zo7zdvnrnt&#10;Owx3LBoqKiQeLTlZNtbNvBl78qQkzFRXy+tOnYCffwZuuMG8czgId/T9330nv2+91fw7/6mpwLRp&#10;xuv6emvSAletkue32hx3CNfS/C1aRo0Kfb18OVBVZU7bdXWyRzt+PDB2rMwtbQyFM4OhQ0Nf19YC&#10;n34aXZuBgMTtDRoEfPKJcTw4dNsU58/hgvO3lBTZP7VqBdmlC3DmjPH69tuBr79uWxs1NcDWrfIH&#10;smKFBIk2pqjIqNRkQ5x/WyQ4f/P5rL1dkZISKtyuXS1/Zvlyme+dPAmcOiV/EMHwpqQkoG9fYP9+&#10;a643Rjh/SN20SX5bNZwGaby5f/x4qICRKC2V56weOAD88488Z3XiRCAvT3rmZ56x7npjhPN7OKvn&#10;b0EiLRJOnWr+wcBTpkhORXKybPg3Lg/hQJwtXEWFDEmpqcD111t7rkjCJSQ0/xmv19i1cAnOHlKD&#10;vdttt1mb+e73h2/oJyQAaWnWndOmuEM4q4fTSBP7K65geYcIUDgz2L49/Njll1t7TpviXOHKy6Xn&#10;SUuTqA4r2bYt/BhLO0TEucIFe7dbbrF+aNu6NfzYAw9Ye06b4nzhrF6dbtsGlJWFHvN6ZaFCwnC+&#10;cFdfbe15liwJP3bffcxHbQJnCldeLnfvAdnjtIq6OiOxOkh8PJNpmsGZwgV7N0CksIr8fODff0OP&#10;TZ1q/TBuY5wv3IkT1pzD7wfmzAk9lpJiVNUkEXG+cFZVD3/9ddlwb8i8edxdaAHnCXf0qDF/AyLf&#10;I4uWlSvDw8inTweeesr8czkM5wkX7N2GDwe6dpUCz2bGlG3eLE+rabh3OnasPJeLtIhzhRs/3khu&#10;eecdc9r+5RepknT2rHEsJwf4/HPeBmklzhVu5Ejg+eclauPDDyV172JRSqT1+UJzCqZNAzZuNK/s&#10;lwtwlnBHj0oeQLduknzSo4cUCrxwQbaaiovb3mZZmeQnzJhhPII8IQH46COptNRSzBsJwVnCBXs3&#10;n88Y4ubMkRuxhw7J8S+/bF1be/dKMeh+/eSx44DsyU6cCPz5J/Dkk2ZfvStwVsRvU+FIixZJgnJe&#10;ntRwGz0amDQJyM2VXjApSfIPiookx6CgIPTWCiC93Pz5UmqfXDyxrTRhMpmZUt9j167I7+/cqdS4&#10;ceHVkBpWQWr4k50ttUL279f7PYIsWhR+TUVFsbkWk3BOD3fkiMzfmstfGDxYSib88YfkjP76q9y8&#10;ramRCI8rr5RI3YwMCWti2VTTcY5wDfMXWso/ve46+SHacc6iQVc4OYkKCke04gzhjhyRFabXa33+&#10;AokKZwgX7N1yc5ma185xlnAcTts9zhBOV8Ea3Zw717pjNsL+wpWVAQcPSoXxrKxYX425RNr7LSnR&#10;fx0mYv/7cE4bTgMB+SNat06CAxoTLOE1bJjc5LYZFC6WlJcbe7OBgAyXfn/oM1cbU1wsAZ+ARKp0&#10;7SqBCh06yAp9wwbrrzsKKFwsCQSk+qXHYzyxMC3NECguLnzVrZR8LhAAzp+XoIT6egk+MKuQtYXY&#10;u8ZvWZmx/3n4cKyvhrQCey8a7Ny7uRR7C7d7t/ymcLbB3kNqVZWkAY4ezVBvm2Bv4YjtsPeQSmwH&#10;hSNaoXBEKxSOaIXCEa1QOKIVCke0QuGIVigc0QqFI1qhcEQrFI5ohcIRrVA4ohUKR7RC4YhWKBzR&#10;CoUjWqFwRCsUjmiFwhGtUDiiFQpHtELhiFYoHNEKhSNaoXBEKxSOaIXCEa1QOKIVCke0QuGIVigc&#10;0QqFI1qhcEQrFI5ohcIRrfwHAYY/UetcCMcAAAAASUVORK5CYII=&#10;"
       id="image1-4"
       x="1104.108"
       y="261.2587" /><image
       width="32.543751"
       height="33.337498"
       preserveAspectRatio="none"
       xlink:href="data:image/png;base64,iVBORw0KGgoAAAANSUhEUgAAAHsAAAB+CAYAAAAECm7MAAAABHNCSVQICAgIfAhkiAAADRlJREFU&#10;eJztnXlsFFUcx79QaEtZSimtFNACQuUUEARBpJabKKAcogZR1MgVFQIxRaIBDYgoQgAlqJHLcDYe&#10;HFYO5RAtZxFUKKccLbRUSqEHbSndn3/8Mpndzm7b3Z3jTWc+yWZ33+z83sx+5/3em/d+700NIiLY&#10;WIKaRh+AjX7YYlsIW2wLYYttIWyxLYQttoWwxbYQttgWwhbbQthiWwhbbAthi20hbLEthC22hTC3&#10;2IWFgJ4jtCYfDTaP2GVlwK5dwOuvA927A5GRgMMBhIYCDz4IvPIKkJQElJZqk/+ZM0CXLnwMZoVE&#10;Jy+PaPZsopgYIi5bFb+aNSP6+mui0lL1jmHdOiKHg+3PmKGeXZ0RV2ynk+iLL4iio6smcvlXixZE&#10;K1YQ3bvn/zFkZBC9+CLbCw7mi8jE1CASsCJKTwfGjQN275bTwsOBhAQgLg5o2RKIiACuXQPOnweS&#10;k4ErVzzbat0a+PBD4LnngBo1qpZ/SQmwaBEwZw63C2JigO++Ax5/PNAzMxajrzYF27cTNWggl9D4&#10;eKLVq4kKCyveLyWFaNAg7yW9c2eipCSiO3e82zhxgmjqVKKoKHm/xx7jEl4NEKtkf/YZkJjIjbEO&#10;HYDFi4G+fX2zsX8/8N57wG+/ed4eFgbExwPNm3OJvXGDvcPZs8C//8q/q1ULmDkTeP99/lwdMPpq&#10;IyKioiKiMWO4JDkcRIsXB97A2rGDS6U/9X1CAlFqqjrnJhBiiC253/btidLS1LX9009EXbtWLnBQ&#10;EB9HcrK6+QuEGG58925g7Vpg6VJ2s1pw6BCwbRtw8CA37PLzgWbNuLH3yCPA88+zW6/GiCG2jS6Y&#10;pwfNJmBssS2ELbaFsMW2ELbYFsIW20LYYlsIW2wLYYttIWyxLYQttoWwxbYQ1WRUvhxFRRzE8Msv&#10;HK6UkwPcvMmhTY0bA127AkOHAg89ZPSR6kr1GvW6fh2YPx9YvpwFr4w+fYBPP2XxrYCRg+mq4XQS&#10;LVlCFBbGgQjR0UQzZxL9+ivRtWtExcVEly8T7drFUTAtW8pBCzVqEM2bZ/QZ6IL5xc7OJurbVxZ5&#10;/nyigoKK9ykuJvroIw4PlkSfMkWf4zUQc4t96hTHhwMcUnTrlm/7z5njHpq0cqUmhykK5hX7/Hmi&#10;Ro1YpEmT/JsMcPcuUceOstjh4UQ5OeofqyCY89brxg1g4EBukM2aBSxbBgQF+W6ndm3gnXfk73l5&#10;HM5cTTFna3z4cODHH4EXXgDWrw/M1uXLHEMuERvLadUQ84m9ciXw2mt8u7R/P1CnTmD27t4FQkLc&#10;006eBNq1C8yugJjLjV+8CEyZwuHGSUmBCw2wK69Z7m84fTpwuwJinh40pxN4+WWO954/H2jRQh27&#10;eXls25XMTHVsC4Z5SvbGjcDvv/McsGnT1LPrSdiqzvY0GeYQ2+nkabcAT/ZTc6Ld8ePKtMaN1bMv&#10;EOYQe906rkd79fJ9Vmdl7N+vTOvQQd08BEH81nhZGdC2LXDuHLB9OzBokHq2S0qAJk14REyiZUue&#10;wlsNEb9kr1/PQnfpoq7QALB5s7vQADBmjLp5CIT4Yq9axe/jx6tve8UK9+916wJvv61+PoIgthvP&#10;zmY3GxLCrebwcPVsHz4M9Ozpfts1bx4wY4Z6eQiG2CU7KYnr7JEj1RW6qIjXTXMVuls3937yaojY&#10;Ym/cyO/Dh6tr99133XvJ4uKArVv9G0wxEeK68exsXgmhdm2OIXM41LG7bRswbJi8NGVsLN9+xcaq&#10;Y19gxO0u3buXBYmPr5rQBQW8lGVoqPc+8y1bgNGjZaFjYjgo0QJCA6KLDXjvRMnO5sDCpCQeICks&#10;lLfVqgXUrw+0bw/068c2tm7l4EJJ6Kee4tZ4o0aanoZIiOvG27UD0tKAAweAHj3ct+XnA23a8EI4&#10;Dgd3uoSHc5+208kNsJMneZCjPGFhLPrkyfqch0CIWbKvX2ehHQ7g0UeV29PSWGgAeOkldvWS6757&#10;F8jKYs+wZQu35l3p1YtXNrYixkRDVcLGjRwTNniw5+3FxURDhnAYcGXrm3XuTJSY6B5JGh9PlJur&#10;7zkJgJglW6qv+/TxvD0khOvgK1eA1FSuv0tL2Y0HBXFPWEwM0LkzEB3N+7Rvz+PhAC91+cwzwJ49&#10;ysCF6ozRV5tH2rThEnj4sLp2p01zL/UWmRwgIV4DLSuLx5PDw3mQQs2Ojps3ObgwP5+/164NHDkC&#10;dOqkXh4CI54b37eP33v3Vr9HKzISmDABWLCAv5eWcujwmjX+2SsqAv75hy/QGzf4Ao2K4pApEe/d&#10;jXYtCiZOZBe7YIE29n/+2d2V16njW2PN6eR1y4cM4X29NQybNyd69VWigwe1OQ8/EM+Nt23L/dap&#10;qTyGrTY3bwING7qnLV0KvPlm5fseOQJMnAgcO8bf4+K4CmjRgu/v09O50ffff+779egBfP658bNF&#10;jb7a3MjM5FIREUFUVqZdPtJsT+k1YEDl+6xaRRQSwr8fMYJo717PvystJdq0iahJE/c8atUi+uAD&#10;dc/DR8QSe8MG/mOGDdM2n/JCREVV/Pv16/me3peHwuTmEnXvrnTvU6cGfvx+IpbYEybwH7Jokbb5&#10;uM7Pll7enkHy119EoaFcMr2VZm/k5nLdXT6vhQsDPwc/EEvs1q35zzh+XNt8GjZUCuDtoS/9+/P2&#10;6dP9yys5WZlXWBjRpUv+H7+fiCO2VF9HRnKLV0uCgpQCZGcrf3fwIG9r2pQoP9///Dp1UuY3bpz/&#10;9vxEnL5CqYv0ySe1nZGRl6ccHAkO5vvj8iQl8fudO7zgzsKFyqlCVUHqpnXl++85lFlHxBPbW3+4&#10;Wpw5o0y7/37PF9gff/B7bi4f3/TpPIPUV3r3Vqbl5cnnrBPWE/vAAWVa06aef3v1qjJtzRou6b7g&#10;bfrvxYu+2QkQMcTOzOQSFxXFo1NakpKiTPM23cdbRGv5aqAy6tblcKnyZGT4ZidAxBBbKtVPPKH9&#10;DErJNbsyapTn3yYkKNO6dwfq1fMtTyLPj3rWeXhVLLE7dtQ2n5QUZWmKjuZGoSc+/hgYMED+3rEj&#10;8O23vuebk+PZG9x3n++2AkCMUS9J7FattM1n9Wpl2ogR3kfXHA5g507g0iUOd2rVyr/SeOqU53Sd&#10;+8qNFzszkx96CnDdphXFxfKkA4mgoKoFHrousOMPO3cq06KieBaKjhjvxl1vP4qLtctnxQrg9m33&#10;tPHjta86iOT7dVdmzND96b1iiZ2To00eeXnA7NnuaRER8moOWrJ5s+y5JJo0MSSUWSyxtVqlaO5c&#10;5RjzvHmee83UpKzM8wU1d646Kz35iu4dtK5cvaoM+1WbH35Q9oVPmqR+Pp5YuFDZJ/7WW/rk7QFj&#10;xV67lv+Anj2J6tXjz6dPq2d/zx454EB6Pf20f+uc+kpaGlHduu55Dx6sT95eMNaNSy782Wc5EBAA&#10;lixRx/bRozxb03WwoVcvYMMG7afmFhZyR43r/LPevYFNm4ydFmzYZUZEFBfHV/yRI+zSg4PZ5QYS&#10;L+508gLy5YMBJ0wgKilR79gryn/0aPe8Bw70HhyhI8aJLdXX9evLrm3WLE6LjSW6cMF3m+npRP36&#10;uf/RwcFEX32l6qFXSGKie/4jR+pzkVUB48SW6uuhQ93TJ0+WAwaSk6tm6+RJbvhI9T7AMWOjRxOd&#10;Pav+sXtj2TJ3oRMTtQ/E8AHjxH7jDc/xWE6nvA3gsKBvvuGSXlTEvyksJDpxgujLL4kSEpQt3gED&#10;iFJT9T2ftWuJatbk/END+btgGCe2VF//+afn7ampHGVaXkjX2Ziur27deO7WmTP6ngcR0ZYtHJAI&#10;8NMNDh3S/xiqgDGTBK5e5eiQyEju7KhocOHvv7lv+dgx/m1BAY9UPfAA24iN5aFRo6bb7Nwpt/rj&#10;4oAdO9RbMVlljBkIcY03q2wU6eGH+SUi+/bxbWNJCS8akJwsTxGuiOxsXrSndWtd10k15j5brxAk&#10;LUlJAYYM4cl9AwfytJ+qCA3wRTFqlEVi0Mwu9tGjvABPQQGvdbptm29Ld504we96P5pC91ZCRgY3&#10;ZKKjhbotqTLHjxM1aMDnMG2af+fQsyfvn5mp/vFVgP4lWyrVCQnmW7H/1CkOU7p1C/jkE57b7es5&#10;3L7Ns0EjIngpEB3Rv4FmVhd+7hzQvz/HkK9eDYwd65+d5cuBe/cMebqQ/mLv2cPvZhL70iVePC8z&#10;k0vjmjVVW62BiIUtLmZvkJUlR8tUe7EzMoALF/gPa9NG16z9JiODV0hMT+fvWVn8ChQDxNa3zjab&#10;C79+nYXWYuaGLbZgjB3LdbUWGCC2vt2lrVqxGz93TvsYcTWIjOQGmdo4HBwEqfPdiH5iZ2TI/dlS&#10;/WejK/q5cbO58GqIfmJLT8azxTYM/dz4rVs8eNC/P690YKM74i16Z6MZxs8IsdENW2wLYYttIWyx&#10;LYQttoWwxbYQttgWwhbbQthiWwhbbAthi20hbLEthC22hbDFthC22Bbif9KdDS5RHSH7AAAAAElF&#10;TkSuQmCC&#10;"
       id="image1-8"
       x="1255.3378"
       y="264.6994" /><image
       width="28.045832"
       height="33.072914"
       preserveAspectRatio="none"
       xlink:href="data:image/png;base64,iVBORw0KGgoAAAANSUhEUgAAAGoAAAB9CAYAAABK8va0AAAABHNCSVQICAgIfAhkiAAACeZJREFU&#10;eJztnWtsFFUUx/9lS4GylrppwyJYhFpFW7FSwUe1FoqBqCC+UINREyMIUVESo/JBiEEJ8RUwJD5i&#10;lShoU42xIEFRqqBFhIrG1FLEoLTQUiyU0rItlT1+OBlnZ7eP2e6dnXvX+0s227nbPefO/Oe+z51N&#10;IiKCRnoGuZ0BjT20UIqghVIELZQiaKEUQQulCFooRdBCKYIWShG0UIqghVIELZQiaKEUQQulCFoo&#10;RUhcoTo6gHgutTnsKzGEOnsW2LoVeOghYMoUwOcDvF5g6FBg/HjggQeA8nKgu9sZ/3V1wKRJnAen&#10;IJVpayNavpzI7yfie7rv19ixRG+/TdTdLS4PGzYQeb1s/5lnxNkNQ02hgkGitWuJMjPtCRT+GjeO&#10;qLSU6J9/Bp6Hhgaie+9leykpfAM4SBKRYjET9fXAgw8C27aZaWlpQHExkJMDZGcD6enAkSPAgQPA&#10;5s3AoUM927r4YuD554G77gKSkuz57+oCXnsNWLGC20G/H/jkE+Daa2M9s75x9DYQzZYtROeea5aM&#10;oiKideuIOjr6/l5VFdGMGb2XsPx8ovJyotOne7fxyy9ETzxBlJFhfu+qq7hkxQF1hHr5ZSKPhy9Q&#10;Xh7R119Hb2P7dha3N8FSU4lmziR65BFu+x59lI/Hj7f+X3Iy0XPPiW3r+kF+oQIBonnz+AJ5vUSr&#10;V8d+gb74gkvDQNq34mKi6mox5xYF8gtlVFm5uUS1tWJtf/45UUFB/+J4PJyPzZvF+o8C+TsT27YB&#10;69cDr78OpKY642PXLmDTJuCHH7gTcuoUMHYsd0yuuAK4+27uNLiI/EJpACTKzMT/AC2UImihFEEL&#10;pQhaKEXQQimCFkoRtFCKoIVSBC2UImihFEELpQjJbmcg7gQCwI4dwFdf8RJ9Swtw/Dgv548aBRQU&#10;ALNmARdd5HZOrbi2wBJvmpqInnySaNgwewuEU6cS7dnjdq7/I/GFCgaJ1qzhZXaAI5eWLuWl/CNH&#10;iDo7if76i2jrVl49zs42xUpKIlq50u0zIKJEF6q5mWjaNFOgVauI2tv7/k5nJ9GLL3IImCHY4sXx&#10;yW8fJK5Qv/3G8XsAL6O3tkb3/RUrrFXhu+86kk27JKZQBw4QjRzJF3jhwoEFWp45QzRxoilUWhpR&#10;S4v4vNok8YQ6dswM71q2LDZb779vLVVLlwrJ4kBIPKHmzOGLes89sdv680+rUFlZsdscIIklVGkp&#10;X9CCgr6jXu3S1RXZba+pid3uAEicmYmDB4HFizmkrLwcGDYsdpuDBwODwi7Rvn2x2x0AiTEzEQwC&#10;99/P8XirVgHjxomx29bGtkNpbBRjO0oSo0SVlQHffQfk5QFLloiz25Modnd9CEZ9oYJB3joDAKtX&#10;A8kCK4mff45MGzVKnP0oUF+oDRu43SgsBKZNE2t7x47ItLw8sT5sonZI89mzwCWXAL//DmzZAsyY&#10;Ic52Vxdw3nk8s26Qnc2b41xA7RL14Ycs0qRJYkUCgM8+s4oEAPPmifURBWoL9d57/D5/vnjbpaXW&#10;4+HDgccfF+/HLq6M3kRw9CjvW0pNJTp5UqztXbuIBg2yDnRdXu5Qt0SVl3MbdccdvDorikCAn0sR&#10;On6aPBl46ilxPgaAukKVlfH7bbeJtfvss9bZh5wcYONGwOMR6ydK1Oz1NTfzDsDBgznmwesVY3fT&#10;JmD2bPNxOVlZ3EXPyhJjPwbUnEL65hu+mEVF9kRqb+fH6wwd2vscYEUFMHeuKZLfzwEwEogEqCwU&#10;0PsAt7kZeOMNbscOHuQHdxgkJwMjRgC5uUBJCdvYuBF46SVTpJtu4l7fyJGOnkY0qFn1XXopUFsL&#10;7NwJXH219bNTp4AJE3jTtNfLA+K0NJ6jCwa5s1BTwxOu4aSmsmCLFsXnPKJAvRJ19CiL5PUCV14Z&#10;+XltLYsEAPfdx9WjUd2dOQM0NXGJrKjgXmMohYX8hDIZcXVwMBDKynhcM3Nmz593dhLdcguHevUX&#10;u5efT/T009aIo6IiohMn4ntONlCvRBnt09SpPX8+ZAi3OYcOAdXV3F51d3PV5/HwDIPfD+TnA5mZ&#10;/J3cXF7PAoDt24FbbwUqKyMXDd3E7TslaiZM4Dv/xx/F2l2yRKqZiHDU6kw0NfF6UFoaT5iKHIQe&#10;Pw5ccAF3RgAeo+3eDVx+uTgfMSBR2bbBt9/y+/XXi58p8PmABQvM4+5u4JVXxPqIAbWE6q99ipWS&#10;Euvxxx8Dra3O+IoSLVQoU6ZYjwMB4IMPnPEVJeoI1dTEk6Xp6dxjcwKfL/IJZhUVzviKEnWEMtqn&#10;oiJnu83p6dbjvXud8xUF6ghVWcnvTlV7BuGTtn//DZw+7axPG6gjlNPtk0FPnYcTJ5z1aQM1xlHG&#10;+Mnn4zvcySDI5OTIOcDmZnMWwyXUKFFGabrhBmdFamuLFCklBcjIcM6nTdQSyulqr64uMm3MGNfC&#10;mEPRQoWyc2dk2ujRzvq0ifxCNTbynZ6RwbPcTlJVFZnmUghzOPILZZSm665zvgr6/vvItDvvdNan&#10;TdQRauJEZ/1UVQENDda0zEzuwEiAOkJdeKGzftati0y7/XbX4/kM5BaqsRHYv5//Hj7cOT+dnWZA&#10;p4HHI1WQi9xCGaUJ4IvpFKWlwMmT1rT5852vbqNAHaFaWpzx0dYGLF9uTUtPN3cxSoI6Qjm1G/2F&#10;F4Bjx6xpK1dKMRthwd2QjT44fDgytEs0n35q/niY8Vq4ULwfAcgr1Pr1fOGuuYbonHP47337xNmv&#10;rCQaMsQq0s03x/YDlQ4ib9VnVHtz5phBJ2vWiLG9Zw/v2ujqMtMKC4GPPpKmOx6B23dKr+Tk8F2+&#10;ezdXgykpXE3FEs8XDPLDE8OfgrlgAT9OR2LkFMpon0aMMKuiZcvMB0f98Uf0NuvriUpKrAKlpBC9&#10;9ZbQrDuFnEIZ7dOsWdb0RYs4ffRo+783WFND9NhjZjtnPIJ07lyi/fvF590h5BTq4Yf5gr76qjU9&#10;GDQ/A4imTyd65x0uYYEA/09HB/9m7ptv8i98hm8MuPFGV371M1bkFMpon/bu7fnz6mqi2bMjRQjd&#10;lRH6mjyZY8nr6uJ7HgKRL2bi8GFeVfX5eCDaV2jYr78CX34J/PQT/297O894n38+28jK4uURSbZ3&#10;xoJ8225C4yP6i9+77DJ+/Q+QbxwVr2V3xdBCKYJcbZTRPmVm8l5dCaJ/ZEGuEmWUpuJiLVIYcgql&#10;q70I5BIqXhsBFESeNqqhgcc/fr9rT0KWGXlKlK72+kQLpQhaKEWQo40y2qcxY4D6erdzIyVylChd&#10;mvpFDqGMJ/ZroXpFjqqvtZWD9KdP5x1+mgjkEErTL3JUfZp+0UIpghZKEbRQiqCFUgQtlCJooRRB&#10;C6UIWihF0EIpghZKEbRQiqCFUoR/AZv0aEsRNLM/AAAAAElFTkSuQmCC&#10;"
       id="image1-16"
       x="1259.7678"
       y="445.86703" /><path
       style="display:inline;opacity:0.512626;fill:none;fill-opacity:1;stroke:#fe0000;stroke-width:0.926042;stroke-dasharray:11.1125, 11.1125;stroke-dashoffset:0;stroke-opacity:1"
       d="m 1257.3396,465.17643 c -9.2117,14.72812 -85.9822,6.34633 -98.7625,1.07095"
       id="path197"
       sodipodi:nodetypes="cc" /></g><g
     id="g134"
     inkscape:label="FLUTE"
     inkscape:export-filename=".\flute.png"
     inkscape:export-xdpi="96"
     inkscape:export-ydpi="96"
     transform="matrix(0.9263812,0,0,1.0004027,-608.16512,-127.68418)"><g
       id="g58"
       inkscape:label="generaINF TYPE"
       style="display:inline;stroke-width:1.4006;stroke-dasharray:none"
       transform="matrix(0.94666662,0,0,0.94241181,163.4309,-78.572482)"
       inkscape:export-filename="..\Documents\TEX FILES\research what am i doing\short curves\fig\rholadder.png"
       inkscape:export-xdpi="96"
       inkscape:export-ydpi="96"><path
         id="path4"
         style="display:inline;fill:url(#linearGradient233);fill-opacity:1;stroke:#000000;stroke-width:1.4006;stroke-dasharray:none;stroke-opacity:1"
         inkscape:label="surface line bottom"
         d="m 521.57359,295.28975 c 0.69257,24.69599 17.26397,62.59702 58.11766,62.82837 40.85369,0.23135 713.80175,-1.64124 713.80175,-1.64124 l 0.768,-128.64019 c 0,0 -677.90576,-0.0989 -720.10291,0.35218 -42.19716,0.45107 -53.27707,42.4049 -52.5845,67.10088 z"
         sodipodi:nodetypes="zzcczz" /><g
         id="g29"
         style="display:none;stroke-width:1.61117;stroke-dasharray:none"
         inkscape:label="double genus"
         transform="matrix(0.92836947,0,0,0.81400337,67.318693,52.198656)"><g
           id="g28"
           inkscape:label="shadow genus together now1"
           style="display:inline;stroke-width:1.61117;stroke-dasharray:none"
           transform="translate(18.432243,1.1572163)"><path
             style="display:none;fill:url(#linearGradient340);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
             id="path7"
             inkscape:label="shadowR"
             sodipodi:nodetypes="cccccc" /><path
             style="display:none;fill:url(#linearGradient341);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
             id="path10"
             inkscape:label="shadowL"
             sodipodi:nodetypes="cccccc" /><path
             style="display:inline;fill:url(#radialGradient341);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
             id="path11"
             inkscape:label="shadowR"
             clip-path="url(#clipPath218)"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)" /><path
             style="display:inline;fill:url(#radialGradient342);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
             id="path18"
             inkscape:label="shadowL purp"
             clip-path="url(#clipPath217)"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)" /><g
             id="g27"
             inkscape:label="genus hole 1"
             style="display:inline;stroke-width:1.63241;stroke-dasharray:none"
             transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
               style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
               id="path26"
               inkscape:path-effect="#path-effect138"
               inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
               sodipodi:nodetypes="cscc"
               transform="translate(311.23778,-33.331065)" /><path
               style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
               id="path27"
               inkscape:path-effect="#path-effect140"
               inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
               sodipodi:nodetypes="cssc"
               transform="translate(310.49613,-35.888171)" /></g></g></g><g
         id="g52"
         style="display:none;stroke-width:1.61117;stroke-dasharray:none"
         inkscape:label="double genus"
         transform="matrix(0.92836947,0,0,0.81400337,277.76424,51.209087)"><g
           id="g41"
           inkscape:label="shadow genus together now"
           style="display:inline;stroke-width:1.61117;stroke-dasharray:none"
           transform="translate(165.3405,1.8294203)"><path
             style="display:none;fill:url(#linearGradient342);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
             id="path29"
             inkscape:label="shadowR"
             sodipodi:nodetypes="cccccc" /><path
             style="display:none;fill:url(#linearGradient343);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
             id="path30"
             inkscape:label="shadowL"
             sodipodi:nodetypes="cccccc" /><path
             style="display:inline;fill:url(#radialGradient343);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
             id="path31"
             inkscape:label="shadowR"
             clip-path="url(#clipPath218)"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)" /><path
             style="display:inline;fill:url(#radialGradient344);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
             id="path37"
             inkscape:label="shadowL purp"
             clip-path="url(#clipPath217)"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)" /><g
             id="g40"
             inkscape:label="genus hole 1"
             style="display:inline;stroke-width:1.63241;stroke-dasharray:none"
             transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
               style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
               id="path38"
               inkscape:path-effect="#path-effect142"
               inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
               sodipodi:nodetypes="cscc"
               transform="translate(311.23778,-33.331065)" /><path
               style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
               id="path39"
               inkscape:path-effect="#path-effect144"
               inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
               sodipodi:nodetypes="cssc"
               transform="translate(310.49613,-35.888171)" /></g></g><g
           id="g51"
           inkscape:label="shadow genus together now1"
           style="display:inline;stroke-width:1.61117;stroke-dasharray:none"
           transform="translate(39.936526,1.9286938)"><path
             style="display:none;fill:url(#linearGradient344);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
             id="path41"
             inkscape:label="shadowR"
             sodipodi:nodetypes="cccccc" /><path
             style="display:none;fill:url(#linearGradient345);fill-opacity:1;stroke:none;stroke-width:1.61117;stroke-dasharray:none"
             d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
             id="path42"
             inkscape:label="shadowL"
             sodipodi:nodetypes="cccccc" /><path
             style="display:inline;fill:url(#radialGradient345);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
             id="path43"
             inkscape:label="shadowR"
             clip-path="url(#clipPath218)"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)" /><path
             style="display:inline;fill:url(#radialGradient346);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
             d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
             id="path44"
             inkscape:label="shadowL purp"
             clip-path="url(#clipPath217)"
             sodipodi:nodetypes="ccccccc"
             transform="matrix(0.974146,0,0,1,21.488772,0)" /><g
             id="g50"
             inkscape:label="genus hole 1"
             style="display:inline;stroke-width:1.63241;stroke-dasharray:none"
             transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
               style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
               id="path45"
               inkscape:path-effect="#path-effect146"
               inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
               sodipodi:nodetypes="cscc"
               transform="translate(311.23778,-33.331065)" /><path
               style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
               d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
               id="path49"
               inkscape:path-effect="#path-effect149"
               inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
               sodipodi:nodetypes="cssc"
               transform="translate(310.49613,-35.888171)" /></g></g></g><g
         id="g57"
         inkscape:label="single genus "
         style="display:none;stroke-width:1.61117;stroke-dasharray:none"
         transform="matrix(0.92836947,0,0,0.81400337,-35.60405,51.707014)"><path
           style="display:inline;fill:url(#radialGradient347);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path53"
           inkscape:label="shadowR"
           clip-path="url(#clipPath218)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><path
           style="display:inline;fill:url(#radialGradient348);fill-opacity:1;stroke:none;stroke-width:1.63241;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path54"
           inkscape:label="shadowL purp"
           clip-path="url(#clipPath217)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><g
           id="g56"
           inkscape:label="genus hole 1"
           style="display:inline;stroke-width:1.63241;stroke-dasharray:none"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path55"
             inkscape:path-effect="#path-effect152"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             sodipodi:nodetypes="cscc"
             transform="translate(311.23778,-33.331065)" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.63241;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path56"
             inkscape:path-effect="#path-effect154"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g></g><g
       id="g83"
       inkscape:label="genus and curve"
       style="display:none"><g
         id="g81"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient348);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path74"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient349);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path75"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient349);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path76"
           inkscape:label="shadowR"
           clip-path="url(#clipPath218)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><path
           style="display:inline;fill:url(#radialGradient350);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path77"
           inkscape:label="shadowL purp"
           clip-path="url(#clipPath217)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><g
           id="g79"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path78"
             inkscape:path-effect="#path-effect168"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             sodipodi:nodetypes="cscc"
             transform="translate(311.23778,-33.331065)" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path79"
             inkscape:path-effect="#path-effect170"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g></g><g
       id="g91"
       inkscape:label="genus and curve"
       transform="translate(146.50048)"
       style="display:none"><g
         id="g89"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient350);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path83"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient351);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path84"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient351);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path85"
           inkscape:label="shadowR"
           clip-path="url(#clipPath218)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><path
           style="display:inline;fill:url(#radialGradient352);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path86"
           inkscape:label="shadowL purp"
           clip-path="url(#clipPath217)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><g
           id="g88"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path87"
             inkscape:path-effect="#path-effect172"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             sodipodi:nodetypes="cscc"
             transform="translate(311.23778,-33.331065)" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path88"
             inkscape:path-effect="#path-effect175"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g></g><g
       id="g105"
       inkscape:label="genus and curve"
       transform="translate(-144.99516)"
       style="display:none"><g
         id="g101"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient352);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path95"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient353);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path96"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient353);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path97"
           inkscape:label="shadowR"
           clip-path="url(#clipPath218)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><path
           style="display:inline;fill:url(#radialGradient354);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path98"
           inkscape:label="shadowL purp"
           clip-path="url(#clipPath217)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><g
           id="g100"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path99"
             inkscape:path-effect="#path-effect178"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             sodipodi:nodetypes="cscc"
             transform="translate(311.23778,-33.331065)" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path100"
             inkscape:path-effect="#path-effect180"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g></g><g
       id="g122"
       inkscape:label="genus and curve"
       transform="translate(291.59808,-0.72704953)"
       style="display:none"><g
         id="g115"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient354);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path105"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient355);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path106"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient355);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path107"
           inkscape:label="shadowR"
           clip-path="url(#clipPath218)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><path
           style="display:inline;fill:url(#radialGradient356);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path108"
           inkscape:label="shadowL purp"
           clip-path="url(#clipPath217)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><g
           id="g114"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path113"
             inkscape:path-effect="#path-effect182"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             sodipodi:nodetypes="cscc"
             transform="translate(311.23778,-33.331065)" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path114"
             inkscape:path-effect="#path-effect184"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g></g><g
       id="g129"
       inkscape:label="genus and curve"
       transform="translate(-290.74719,-0.08063906)"
       style="display:none"><g
         id="g128"
         inkscape:label="single genus"
         style="display:inline"
         transform="matrix(0.87885638,0,0,0.76712639,353.74228,-26.040516)"><path
           style="display:none;fill:url(#linearGradient356);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 795.21683,284.76823 30.94202,-9.2965 4.68195,-9.43357 -7.81189,19.68071 -9.1582,8.65406 z"
           id="path122"
           inkscape:label="shadowR"
           sodipodi:nodetypes="cccccc" /><path
           style="display:none;fill:url(#linearGradient357);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 775.76627,284.38248 -30.94202,-9.2965 -4.68195,-9.43357 7.81189,19.68071 9.1582,8.65406 z"
           id="path123"
           inkscape:label="shadowL"
           sodipodi:nodetypes="cccccc" /><path
           style="display:inline;fill:url(#radialGradient357);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 784.3988,283.80387 43.23019,-6.01772 3.52993,-12.13374 -7.81189,19.68071 -9.1582,8.65406 -17.5708,-8.15597 z"
           id="path124"
           inkscape:label="shadowR"
           clip-path="url(#clipPath218)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><path
           style="display:inline;fill:url(#radialGradient358);fill-opacity:1;stroke:none;stroke-width:0;stroke-dasharray:none"
           d="m 785.82663,284.02983 -43.23019,-6.01772 -3.52993,-12.13374 7.81189,19.68071 9.1582,8.65406 17.5708,-8.15597 z"
           id="path125"
           inkscape:label="shadowL purp"
           clip-path="url(#clipPath217)"
           sodipodi:nodetypes="ccccccc"
           transform="matrix(0.974146,0,0,1,21.488772,0)" /><g
           id="g127"
           inkscape:label="genus hole 1"
           style="display:inline"
           transform="matrix(0.974146,0,0,1,227.64799,-321.21397)"><path
             style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 234.41965,648.83801 c 6.23479,-5.35812 14.03742,-8.8694 22.18256,-9.98243 8.14514,-1.11303 16.60375,0.17616 24.04749,3.66511 3.76844,1.7663 7.27796,4.08387 10.38217,6.85602 v 0"
             id="path126"
             inkscape:path-effect="#path-effect186"
             inkscape:original-d="m 234.41965,648.83801 c 13.01832,-12.41928 30.02179,-13.39667 46.23005,-6.31732 3.47131,1.51617 7.38862,7.94454 10.38217,6.85602 3.07789,7.33132 2.16595,3.13365 0,0"
             sodipodi:nodetypes="cscc"
             transform="translate(311.23778,-33.331065)" /><path
             style="display:inline;opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:none;stroke-opacity:1"
             d="m 221.68681,636.69307 c 3.18403,5.13639 7.18335,9.76623 11.80236,13.66307 3.43991,2.9021 7.22986,5.4031 11.31265,7.29676 11.26493,5.22485 24.71052,5.52936 36.20045,0.81986 11.48992,-4.70949 20.85384,-14.36318 25.21108,-25.99126"
             id="path127"
             inkscape:path-effect="#path-effect190"
             inkscape:original-d="m 221.68681,636.69307 c 1.8773,11.71999 2.21846,7.89328 11.80236,13.66307 3.85908,2.32326 7.03622,5.70111 11.31265,7.29676 23.09698,8.61812 47.43322,-7.46588 61.41153,-25.1714"
             sodipodi:nodetypes="cssc"
             transform="translate(310.49613,-35.888171)" /></g></g></g></g><g
     id="g283"
     inkscape:label="punctures"
     transform="translate(-257.85719,-126.78496)"
     inkscape:export-filename=".\flute.png"
     inkscape:export-xdpi="96"
     inkscape:export-ydpi="96"><g
       id="g280"
       transform="matrix(0.53712513,0.53386543,-0.53386543,0.53712513,446.42137,-348.56948)"
       inkscape:label="punct"><path
         style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
         d="M 740.82049,231.21722 H 767.1682"
         id="path279"
         inkscape:path-effect="#path-effect288"
         inkscape:original-d="M 740.82049,231.21722 H 767.1682" /><path
         style="fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
         d="M 740.82049,231.21722 H 767.1682"
         id="path280"
         inkscape:path-effect="#path-effect290"
         inkscape:original-d="M 740.82049,231.21722 H 767.1682"
         transform="rotate(-90.06457,754.18558,231.20967)" /></g><g
       id="g260"
       inkscape:label="punctures"
       transform="translate(-397.02306)"><g
         id="g208"
         transform="matrix(0.53712513,0.53386543,-0.53386543,0.53712513,511.62589,-348.85928)"
         inkscape:label="punct"><path
           style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path208"
           inkscape:path-effect="#path-effect208"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682" /><path
           style="fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path208-8"
           inkscape:path-effect="#path-effect208-4"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682"
           transform="rotate(-90.06457,754.18558,231.20967)" /></g><g
         id="g253"
         transform="matrix(0.53712513,0.53386543,-0.53386543,0.53712513,446.42137,-348.56948)"
         inkscape:label="punct"><path
           style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path252"
           inkscape:path-effect="#path-effect254"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682" /><path
           style="fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path253"
           inkscape:path-effect="#path-effect256"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682"
           transform="rotate(-90.06457,754.18558,231.20967)" /></g><g
         id="g257"
         transform="matrix(0.53712513,0.53386543,-0.53386543,0.53712513,578.27939,-348.85928)"
         inkscape:label="punct"><path
           style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path256"
           inkscape:path-effect="#path-effect258"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682" /><path
           style="fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path257"
           inkscape:path-effect="#path-effect260"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682"
           transform="rotate(-90.06457,754.18558,231.20967)" /></g></g><g
       id="g266"
       inkscape:label="punctures"
       transform="translate(-198.22173)"><g
         id="g261"
         transform="matrix(0.53712513,0.53386543,-0.53386543,0.53712513,511.62589,-348.85928)"
         inkscape:label="punct"><path
           style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path260"
           inkscape:path-effect="#path-effect267"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682" /><path
           style="fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path261"
           inkscape:path-effect="#path-effect269"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682"
           transform="rotate(-90.06457,754.18558,231.20967)" /></g><g
         id="g263"
         transform="matrix(0.53712513,0.53386543,-0.53386543,0.53712513,446.42137,-348.56948)"
         inkscape:label="punct"><path
           style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path262"
           inkscape:path-effect="#path-effect271"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682" /><path
           style="fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path263"
           inkscape:path-effect="#path-effect273"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682"
           transform="rotate(-90.06457,754.18558,231.20967)" /></g><g
         id="g265"
         transform="matrix(0.53712513,0.53386543,-0.53386543,0.53712513,578.27939,-348.85928)"
         inkscape:label="punct"><path
           style="opacity:1;fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path264"
           inkscape:path-effect="#path-effect275"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682" /><path
           style="fill:none;fill-opacity:1;stroke:#000000;stroke-width:0.79375;stroke-dasharray:none;stroke-opacity:1"
           d="M 740.82049,231.21722 H 767.1682"
           id="path265"
           inkscape:path-effect="#path-effect277"
           inkscape:original-d="M 740.82049,231.21722 H 767.1682"
           transform="rotate(-90.06457,754.18558,231.20967)" /></g></g></g><path
     style="opacity:1;fill:#fdfdfd;fill-opacity:1;stroke:#000000;stroke-width:1.32292;stroke-dasharray:1.32292, 31.75;stroke-dashoffset:0;stroke-opacity:1"
     d="m 1302.9312,159.96842 70.7107,-0.5796"
     id="path339"
     inkscape:path-effect="#path-effect339"
     inkscape:original-d="m 1302.9312,159.96842 70.7107,-0.5796"
     transform="translate(-768.58045,-110.33326)" /></svg>

